Constant-delay enumeration for SLP-compressed documents

We study the problem of enumerating results from a query over a compressed document. The model we use for compression are straight-line programs (SLPs), which are defined by a context-free grammar that produces a single string. For our queries, we use a model called Annotated Automata, an extension of regular automata that allows annotations on letters. This model extends the notion of Regular Spanners as it allows arbitrarily long outputs. Our main result is an algorithm that evaluates such a query by enumerating all results with output-linear delay after a preprocessing phase which takes linear time on the size of the SLP, and cubic time over the size of the automaton. This is an improvement over Schmid and Schweikardt's result, which, with the same preprocessing time, enumerates with a delay that is logarithmic on the size of the uncompressed document. We achieve this through a persistent data structure named Enumerable Compact Sets with Shifts which guarantees output-linear delay under certain restrictions. These results imply constant-delay enumeration algorithms in the context of regular spanners. Further, we use an extension of annotated automata which utilizes succinctly encoded annotations to save an exponential factor from previous results that dealt with constant-delay enumeration over vset automata. Lastly, we extend our results in the same fashion Schmid and Schweikardt did to allow complex document editing while maintaining the constant delay guarantee.

==> figures/enumfig.tex <==
%!TEX root = ../../main.tex

\begin{tikzpicture}[->,>=stealth',roundnode/.style={circle,draw,inner sep=1.2pt},squarednode/.style={rectangle,inner sep=3pt}]
	
	\node [squarednode] (0) at (1, 0) {$a_3$};
%	\node [roundnode] (0b) at (1, 0.3) {};
	\node [squarednode] (1) at (3, 0) {$a_4$};
%	\node [roundnode] (1b) at (3, 0.3) {};
	\node [squarednode] (2) at (2, 1) {$\cup$};
%	\node [roundnode] (2b) at (2, 1.3) {};
	\node [squarednode] (3) at (0, 1) {$a_2$};
%	\node [roundnode] (3b) at (0, 1.3) {};
	\node [squarednode] (4) at (1, 2) {$\cup$};
%	\node [roundnode] (4b) at (1, 2.3) {};
	\node [squarednode] (5) at (3, 2) {$a_5$};
%	\node [roundnode] (5b) at (3, 2.3) {};
	\node [squarednode] (6) at (2, 3) {$\cup$};
%	\node [roundnode] (6b) at (2, 3.3) {};
	\node [squarednode] (7) at (0, 3) {$a_1$};
	\node [roundnode] (7b) at (0, 3.3) {};
	\node [squarednode] (8) at (1, 4) {$\cup$};
	\node [roundnode] (8b) at (1, 4.3) {};
	\node [squarednode] (9) at (3, 4) {$a_6$};
%	\node [roundnode] (9b) at (3, 4.3) {};
	\node [squarednode] (10) at (2, 5) {$\cup$};
	\node [roundnode] (10b) at (2, 5.3) {};
	\node [squarednode] (11) at (0, 5) {$\ldots$};
	\node [squarednode] (12) at (1, 6) {$\odot$};
%	\node [roundnode] (12b) at (1, 6.3) {};
	
	\draw (2) to (0);
	\draw (2) to (1);
	\draw (4) to (2);
	\draw (4) to (3);
	\draw (6) to (4);
	\draw (6) to (5);
	\draw (8) to (6);
	\draw (8) to (7);
	\draw (10) to (8);
	\draw (10) to (9);
	\draw (12) to (10);
	\draw (12) to (11);
	
%	\draw[dashed, -, out=200, in=70] (12b) to (10b);
	\draw[dashed, -, out=200, in=70] (10b) to (8b);
	\draw[dashed, -, out=200, in=70] (8b) to (7b);
%	\draw[dashed, -, out=200, in=110] (10b) to (6b);
%	\draw[dashed, -, out=200, in=70] (6b) to (4b);
%	\draw[dashed, -, out=200, in=70] (4b) to (3b);
%	\draw[dashed, -, out=200, in=110] (6b) to (2b);
%	\draw[dashed, -, out=200, in=70] (2b) to (0b);
%	\draw[dashed, -, out=200, in=110] (6b) to (1b);
%	\draw[dashed, -, out=200, in=110] (10b) to (5b);
%	\draw[dashed, -, out=200, in=110] (12b) to (9b);

\end{tikzpicture}
\begin{tikzpicture}[->,>=stealth',roundnode/.style={circle,draw,inner sep=1.2pt},squarednode/.style={rectangle,inner sep=3pt}]
	
	\node [squarednode] (0) at (1, 0) {$a_3$};
%	\node [roundnode] (0b) at (1, 0.3) {};
	\node [squarednode] (1) at (3, 0) {$a_4$};
%	\node [roundnode] (1b) at (3, 0.3) {};
	\node [squarednode] (2) at (2, 1) {$\cup$};
%	\node [roundnode] (2b) at (2, 1.3) {};
	\node [squarednode] (3) at (0, 1) {$a_2$};
	\node [roundnode] (3b) at (0, 1.3) {};
	\node [squarednode] (4) at (1, 2) {$\cup$};
	\node [roundnode] (4b) at (1, 2.3) {};
	\node [squarednode] (5) at (3, 2) {$a_5$};
%	\node [roundnode] (5b) at (3, 2.3) {};
	\node [squarednode] (6) at (2, 3) {$\cup$};
	\node [roundnode] (6b) at (2, 3.3) {};
	\node [squarednode] (7) at (0, 3) {$a_1$};
%	\node [roundnode] (7b) at (0, 3.3) {};
	\node [squarednode] (8) at (1, 4) {$\cup$};
%	\node [roundnode] (8b) at (1, 4.3) {};
	\node [squarednode] (9) at (3, 4) {$a_6$};
%	\node [roundnode] (9b) at (3, 4.3) {};
	\node [squarednode] (10) at (2, 5) {$\cup$};
	\node [roundnode] (10b) at (2, 5.3) {};
	\node [squarednode] (11) at (0, 5) {$\ldots$};
	\node [squarednode] (12) at (1, 6) {$\odot$};
	%	\node [roundnode] (12b) at (1, 6.3) {};
	
	\draw (2) to (0);
	\draw (2) to (1);
	\draw (4) to (2);
	\draw (4) to (3);
	\draw (6) to (4);
	\draw (6) to (5);
	\draw (8) to (6);
	\draw (8) to (7);
	\draw (10) to (8);
	\draw (10) to (9);
	\draw (12) to (10);
	\draw (12) to (11);
	
%	\draw[dashed, -, out=200, in=70] (12b) to (10b);
%	\draw[dashed, -, out=200, in=70] (10b) to (8b);
%	\draw[dashed, -, out=200, in=70] (8b) to (7b);
	\draw[dashed, -, out=200, in=110] (10b) to (6b);
	\draw[dashed, -, out=200, in=70] (6b) to (4b);
	\draw[dashed, -, out=200, in=70] (4b) to (3b);
%	\draw[dashed, -, out=200, in=110] (6b) to (2b);
%	\draw[dashed, -, out=200, in=70] (2b) to (0b);
%	\draw[dashed, -, out=200, in=110] (6b) to (1b);
%	\draw[dashed, -, out=200, in=110] (10b) to (5b);
%	\draw[dashed, -, out=200, in=110] (12b) to (9b);
\end{tikzpicture}
\begin{tikzpicture}[->,>=stealth',roundnode/.style={circle,draw,inner sep=1.2pt},squarednode/.style={rectangle,inner sep=3pt}]
	
	\node [squarednode] (0) at (1, 0) {$a_3$};
	\node [roundnode] (0b) at (1, 0.3) {};
	\node [squarednode] (1) at (3, 0) {$a_4$};
%	\node [roundnode] (1b) at (3, 0.3) {};
	\node [squarednode] (2) at (2, 1) {$\cup$};
	\node [roundnode] (2b) at (2, 1.3) {};
	\node [squarednode] (3) at (0, 1) {$a_2$};
%	\node [roundnode] (3b) at (0, 1.3) {};
	\node [squarednode] (4) at (1, 2) {$\cup$};
%	\node [roundnode] (4b) at (1, 2.3) {};
	\node [squarednode] (5) at (3, 2) {$a_5$};
%	\node [roundnode] (5b) at (3, 2.3) {};
	\node [squarednode] (6) at (2, 3) {$\cup$};
	\node [roundnode] (6b) at (2, 3.3) {};
	\node [squarednode] (7) at (0, 3) {$a_1$};
%	\node [roundnode] (7b) at (0, 3.3) {};
	\node [squarednode] (8) at (1, 4) {$\cup$};
%	\node [roundnode] (8b) at (1, 4.3) {};
	\node [squarednode] (9) at (3, 4) {$a_6$};
%	\node [roundnode] (9b) at (3, 4.3) {};
	\node [squarednode] (10) at (2, 5) {$\cup$};
	\node [roundnode] (10b) at (2, 5.3) {};
	\node [squarednode] (11) at (0, 5) {$\ldots$};
	\node [squarednode] (12) at (1, 6) {$\odot$};
	%	\node [roundnode] (12b) at (1, 6.3) {};
	
	\draw (2) to (0);
	\draw (2) to (1);
	\draw (4) to (2);
	\draw (4) to (3);
	\draw (6) to (4);
	\draw (6) to (5);
	\draw (8) to (6);
	\draw (8) to (7);
	\draw (10) to (8);
	\draw (10) to (9);
	\draw (12) to (10);
	\draw (12) to (11);
	
%	\draw[dashed, -, out=200, in=70] (12b) to (10b);
%	\draw[dashed, -, out=200, in=70] (10b) to (8b);
%	\draw[dashed, -, out=200, in=70] (8b) to (7b);
	\draw[dashed, -, out=200, in=110] (10b) to (6b);
%	\draw[dashed, -, out=200, in=70] (6b) to (4b);
%	\draw[dashed, -, out=200, in=70] (4b) to (3b);
	\draw[dashed, -, out=200, in=110] (6b) to (2b);
	\draw[dashed, -, out=200, in=70] (2b) to (0b);
%	\draw[dashed, -, out=200, in=110] (6b) to (1b);
%	\draw[dashed, -, out=200, in=110] (10b) to (5b);
%	\draw[dashed, -, out=200, in=110] (12b) to (9b);
\end{tikzpicture}

\vspace{1em}

\begin{tikzpicture}[->,>=stealth',roundnode/.style={circle,draw,inner sep=1.2pt},squarednode/.style={rectangle,inner sep=3pt}]
	
	\node [squarednode] (0) at (1, 0) {$a_3$};
%	\node [roundnode] (0b) at (1, 0.3) {};
	\node [squarednode] (1) at (3, 0) {$a_4$};
	\node [roundnode] (1b) at (3, 0.3) {};
	\node [squarednode] (2) at (2, 1) {$\cup$};
%	\node [roundnode] (2b) at (2, 1.3) {};
	\node [squarednode] (3) at (0, 1) {$a_2$};
%	\node [roundnode] (3b) at (0, 1.3) {};
	\node [squarednode] (4) at (1, 2) {$\cup$};
%	\node [roundnode] (4b) at (1, 2.3) {};
	\node [squarednode] (5) at (3, 2) {$a_5$};
%	\node [roundnode] (5b) at (3, 2.3) {};
	\node [squarednode] (6) at (2, 3) {$\cup$};
	\node [roundnode] (6b) at (2, 3.3) {};
	\node [squarednode] (7) at (0, 3) {$a_1$};
%	\node [roundnode] (7b) at (0, 3.3) {};
	\node [squarednode] (8) at (1, 4) {$\cup$};
%	\node [roundnode] (8b) at (1, 4.3) {};
	\node [squarednode] (9) at (3, 4) {$a_6$};
%	\node [roundnode] (9b) at (3, 4.3) {};
	\node [squarednode] (10) at (2, 5) {$\cup$};
	\node [roundnode] (10b) at (2, 5.3) {};
	\node [squarednode] (11) at (0, 5) {$\ldots$};
	\node [squarednode] (12) at (1, 6) {$\odot$};
	%	\node [roundnode] (12b) at (1, 6.3) {};
	
	\draw (2) to (0);
	\draw (2) to (1);
	\draw (4) to (2);
	\draw (4) to (3);
	\draw (6) to (4);
	\draw (6) to (5);
	\draw (8) to (6);
	\draw (8) to (7);
	\draw (10) to (8);
	\draw (10) to (9);
	\draw (12) to (10);
	\draw (12) to (11);
	
%	\draw[dashed, -, out=200, in=70] (12b) to (10b);
%	\draw[dashed, -, out=200, in=70] (10b) to (8b);
%	\draw[dashed, -, out=200, in=70] (8b) to (7b);
	\draw[dashed, -, out=200, in=110] (10b) to (6b);
%	\draw[dashed, -, out=200, in=70] (6b) to (4b);
%	\draw[dashed, -, out=200, in=70] (4b) to (3b);
%	\draw[dashed, -, out=200, in=110] (6b) to (2b);
%	\draw[dashed, -, out=200, in=70] (2b) to (0b);
	\draw[dashed, -, out=200, in=110] (6b) to (1b);
%	\draw[dashed, -, out=200, in=110] (10b) to (5b);
%	\draw[dashed, -, out=200, in=110] (12b) to (9b);
\end{tikzpicture}
\begin{tikzpicture}[->,>=stealth',roundnode/.style={circle,draw,inner sep=1.2pt},squarednode/.style={rectangle,inner sep=3pt}]
	
	\node [squarednode] (0) at (1, 0) {$a_3$};
%	\node [roundnode] (0b) at (1, 0.3) {};
	\node [squarednode] (1) at (3, 0) {$a_4$};
%	\node [roundnode] (1b) at (3, 0.3) {};
	\node [squarednode] (2) at (2, 1) {$\cup$};
%	\node [roundnode] (2b) at (2, 1.3) {};
	\node [squarednode] (3) at (0, 1) {$a_2$};
%	\node [roundnode] (3b) at (0, 1.3) {};
	\node [squarednode] (4) at (1, 2) {$\cup$};
%	\node [roundnode] (4b) at (1, 2.3) {};
	\node [squarednode] (5) at (3, 2) {$a_5$};
	\node [roundnode] (5b) at (3, 2.3) {};
	\node [squarednode] (6) at (2, 3) {$\cup$};
%	\node [roundnode] (6b) at (2, 3.3) {};
	\node [squarednode] (7) at (0, 3) {$a_1$};
%	\node [roundnode] (7b) at (0, 3.3) {};
	\node [squarednode] (8) at (1, 4) {$\cup$};
%	\node [roundnode] (8b) at (1, 4.3) {};
	\node [squarednode] (9) at (3, 4) {$a_6$};
%	\node [roundnode] (9b) at (3, 4.3) {};
	\node [squarednode] (10) at (2, 5) {$\cup$};
	\node [roundnode] (10b) at (2, 5.3) {};
	\node [squarednode] (11) at (0, 5) {$\ldots$};
	\node [squarednode] (12) at (1, 6) {$\odot$};
	%	\node [roundnode] (12b) at (1, 6.3) {};
	
	\draw (2) to (0);
	\draw (2) to (1);
	\draw (4) to (2);
	\draw (4) to (3);
	\draw (6) to (4);
	\draw (6) to (5);
	\draw (8) to (6);
	\draw (8) to (7);
	\draw (10) to (8);
	\draw (10) to (9);
	\draw (12) to (10);
	\draw (12) to (11);
	
%	\draw[dashed, -, out=200, in=70] (12b) to (10b);
%	\draw[dashed, -, out=200, in=70] (10b) to (8b);
%	\draw[dashed, -, out=200, in=70] (8b) to (7b);
%	\draw[dashed, -, out=200, in=110] (10b) to (6b);
%	\draw[dashed, -, out=200, in=70] (6b) to (4b);
%	\draw[dashed, -, out=200, in=70] (4b) to (3b);
%	\draw[dashed, -, out=200, in=110] (6b) to (2b);
%	\draw[dashed, -, out=200, in=70] (2b) to (0b);
%	\draw[dashed, -, out=200, in=110] (6b) to (1b);
	\draw[dashed, -, out=200, in=110] (10b) to (5b);
%	\draw[dashed, -, out=200, in=110] (12b) to (9b);
\end{tikzpicture}
\begin{tikzpicture}[->,>=stealth',roundnode/.style={circle,draw,inner sep=1.2pt},squarednode/.style={rectangle,inner sep=3pt}]

\node [squarednode] (0) at (1, 0) {$a_3$};
%\node [roundnode] (0b) at (1, 0.3) {};
\node [squarednode] (1) at (3, 0) {$a_4$};
%\node [roundnode] (1b) at (3, 0.3) {};
\node [squarednode] (2) at (2, 1) {$\cup$};
%\node [roundnode] (2b) at (2, 1.3) {};
\node [squarednode] (3) at (0, 1) {$a_2$};
%\node [roundnode] (3b) at (0, 1.3) {};
\node [squarednode] (4) at (1, 2) {$\cup$};
%\node [roundnode] (4b) at (1, 2.3) {};
\node [squarednode] (5) at (3, 2) {$a_5$};
%\node [roundnode] (5b) at (3, 2.3) {};
\node [squarednode] (6) at (2, 3) {$\cup$};
%\node [roundnode] (6b) at (2, 3.3) {};
\node [squarednode] (7) at (0, 3) {$a_1$};
%\node [roundnode] (7b) at (0, 3.3) {};
\node [squarednode] (8) at (1, 4) {$\cup$};
%\node [roundnode] (8b) at (1, 4.3) {};
\node [squarednode] (9) at (3, 4) {$a_6$};
\node [roundnode] (9b) at (3, 4.3) {};
\node [squarednode] (10) at (2, 5) {$\cup$};
%\node [roundnode] (10b) at (2, 5.3) {};
\node [squarednode] (11) at (0, 5) {$\ldots$};
\node [squarednode] (12) at (1, 6) {$\odot$};
%	\node [roundnode] (12b) at (1, 6.3) {};

\draw (2) to (0);
\draw (2) to (1);
\draw (4) to (2);
\draw (4) to (3);
\draw (6) to (4);
\draw (6) to (5);
\draw (8) to (6);
\draw (8) to (7);
\draw (10) to (8);
\draw (10) to (9);
\draw (12) to (10);
\draw (12) to (11);

%\draw[dashed, -, out=200, in=70] (12b) to (10b);
%\draw[dashed, -, out=200, in=70] (10b) to (8b);
%\draw[dashed, -, out=200, in=70] (8b) to (7b);
%\draw[dashed, -, out=200, in=110] (10b) to (6b);
%\draw[dashed, -, out=200, in=70] (6b) to (4b);
%\draw[dashed, -, out=200, in=70] (4b) to (3b);
%\draw[dashed, -, out=200, in=110] (6b) to (2b);
%\draw[dashed, -, out=200, in=70] (2b) to (0b);
%\draw[dashed, -, out=200, in=110] (6b) to (1b);
%\draw[dashed, -, out=200, in=110] (10b) to (5b);
%\draw[dashed, -, out=200, in=110] (12b) to (9b);
\end{tikzpicture}

==> sections/ecsnew.tex <==
%!TEX root = ../main.tex

In this section, we present the data structure, called \emph{Enumerable Compact Sets with Shifts}, that will be used to compactly store the outputs of evaluating an annotated automaton over a straight-line program. This structure extends Enumerable Compact Sets (ECS) introduced in~\cite{MunozR22} (which were, in turn, strongly inspired by the work in~\cite{AmarilliBJM17,AmarilliBMN19}). Indeed, people have also used ECS extensions in~\cite{AmarilliJMR22,BucchiGQRV22}. This new version extends ECS by introducing a shift operator, which allows to succinctly move all outputs' positions with a single call. Although the shift nodes require a revision of the complete ECS model, it simplifies the evaluation algorithm in Section~\ref{sec:evaluation} and achieves output-linear delay for enumerating all the outputs. For completeness of presentation, this section goes through all main details of ECS, as it was done in~\cite{MunozR22}, and how to modify them with shifts. 
%We will follow a preprint of the full version of~\cite{MunozR22} as base of this section~\cite{MunozR22Arxiv}.

\paragraph{The structure} Let $\infAlph$ be an output alphabet such that $\infAlph$ has no elements in common with $\int$ or $\{\cup,\odot\}$ (i.e., $\infAlph \cap \int = \emptyset$ and $\infAlph \cap \{\cup,\odot\} = \emptyset$).
We define an \emph{\dsnamebigcaps{}} (\dsabbr) as a tuple:
\[
\cD \ = \  (\infAlph, V, \lch, \rch, \lambda)
\]
such that $V$ is a finite sets of nodes,
$\lch\colon V \to V$ and $\rch\colon V \to V$ are the {\em left} and {\em right} partial functions, and $\lambda\colon V\to\infAlph \cup \int \cup\{\cup,\odot\}$ is a labeling function.
We call $\ell(v)$ and $r(v)$ the \emph{children} of $v$.
Intuitively, a node defines a set of outputs, and its label indicates how they are formed: whether it utilizes the outputs from its children, and how.
We assume that $\cD$ forms a directed acyclic graph, namely, the induced graph $(V, \{(v,\lch(v)),(v,\rch(v))\mid v\in V\})$ is acyclic. 
Further, for every node $v \in V$, $\lch(v)$ is defined iff  $\lambda(v)\in \int \cup \{\cup, \odot\}$, and $\rch(v)$ is defined iff $\lambda(v)\in \{\cup, \odot\}$.
%Also, we will assume that if $\ell(v) = u$, then $\lambda(u)\not\in\int$.
% This last assumption implies that chains of $\int$-nodes are not allowed.
Notice that, by definition, nodes labeled by $\infAlph$ are bottom nodes in the acyclic structure formed by $\cD$, and nodes labeled by $\int$ or $\{\cup, \odot\}$ are inner nodes. Here, $\int$-nodes are unary operators (i.e., $\rch(\cdot)$ is not defined over them), and $\cup$-nodes or $\odot$-nodes are binary operators. 
Indeed, we say that $v \in V$ is a \textdef{bottom node} if $\lambda(v) \in \infAlph$, a \textdef{product node} if $\lambda(v) = \odot$, a \textdef{union node} if $\lambda(v) = \cup$, and a \textdef{shift node} if $\lambda(v)\in\int$. 
Furthermore, we say that a node is an \textdef{output node} if it is a bottom or product node. 
Finally, we define the size of $\cD$ as $|\cD| = |V|$.

The outputs retrieved from a \dsabbr are strings of the form $(\oout_1, i_1)(\oout_2, i_2)\ldots(\oout_\ell, i_\ell)$, where $\oout_j\in\infAlph$ and $i_j\in\int$.
To build them, we use the {\em shifting function} $\shift: (\infAlph \times \int) \times \int \to (\infAlph \times \int)$ such that $\shift((\oout, i), s) = (\oout, i+s)$.
We extend this function to strings over $\infAlph \times \int$ such that $\shift((\oout_1, i_1)\ldots(\oout_\ell, i_\ell), s) = (\oout_1, i_1+s)\ldots(\oout_\ell, i_\ell+s)$ and to set of strings such that $\shift(L, s) = \{\shift(w, s) \mid w \in L\}$ for every $L \subseteq (\infAlph \times \int)^*$.

As we mentioned, each node $v \in V$ of a \dsabbr $\cD = (\infAlph, V, \lch, \rch, \lambda)$ defines a set of output strings. Specifically, we associate a set of strings $\sem{\cD}(v)$ recursively as follows. For any two sets of strings $L_1$ and $L_2$, define $L_1 \cdot L_2 = \{w_1\cdot w_2 \mid w_1\in L_1\text{ and }w_2\in L_2\}$. Then: 
\begin{itemize}
	\item if $\lambda(v) = \oout \in \infAlph$, then $\sem{\cD}(v) = \{(\oout, 1)\}$;
	\item if $\lambda(v) = \cup$, then $\sem{\cD}(v) = \sem{\cD}(\lch(v)) \cup \sem{\cD}(\rch(v))$;
	\item if $\lambda(v) = \odot$, then $\sem{\cD}(v) = \sem{\cD}(\lch(v)) \cdot \sem{\cD}(\rch(v))$; and 
	\item if $\lambda(v) \in \int$, then $\sem{\cD}(v) = \shift(\sem{\cD}(\lch(v)), \lambda(v))$.
\end{itemize}

\begin{exa}\label{exa:fig}
Suppose $\infAlph = \{x, y\}$. 
Consider the \dsabbr $\cD = (\infAlph, V, \lch, \rch, \lambda)$ where $V = \{v_1, v_2, v_3, v_4, v_5\}$, $\lch(v_1) = v_4$, $\rch(v_1) = v_2$, $\lch(v_2) = v_3$, $\lch(v_3) = v_4$, $\rch(v_3) = v_5$, $\lambda(v_1) = \odot$, $\lambda(v_2) = +2$, $\lambda(v_3) = \cup$, $\lambda(v_4) = x$ and $\lambda(v_5) = y$. 
We show an illustration of this \dsabbr in Figure~\ref{fig-ecsex}. One can easily check that the sets of words $\sem{\cD}$ associated to each node are: 
\[
\begin{array}{rcl}
	\sem{\cD}(v_4) & = & \{(x, 1)\} \\  \sem{\cD}(v_5) & = & \{(y, 1)\} \\ \sem{\cD}(v_3) & = & \{(x, 1), (y, 1)\} \\ \sem{\cD}(v_2) & = & \{(x, 3), (y, 3)\} \\
	\sem{\cD}(v_1) & = & \{(x, 1)(x, 3), (x, 1)(y, 3)\}.
\end{array}
\]
\end{exa}
% \cristian{Ahora que tenemos espacio, yo traería la figura 3(a) a esta página y la removería de la figura 3. La figura 3 quedará un poco desbalanceada, no será tan terrible, pero ganaremos que para el lector es más fácil de verificar el ejemplo.}

% \begin{figure}[t]
% 	\centering
% 	\begin{tikzpicture}[every label/.style={black!60}, ->,>=stealth',roundnode/.style={circle,inner sep=1pt},squarednode/.style={rectangle,inner sep=2pt}, scale=0.85]
		

% 		\node [roundnode, label=180:\footnotesize{$v_4\!:$}] (4) at (0, 0) {$x$};
% 		\node [roundnode, label=180:\footnotesize{$v_5\!:$}] (5) at (4, 0) {$y$};
% 		\node [squarednode, label=180:\footnotesize{$v_3\!:$}] (3) at (2, 1) {$\cup$};
% 		\node [squarednode, label=180:\footnotesize{$v_2\!:$}] (2) at (3, 2) {$+2\ $};
% 		\node [squarednode, label=180:\footnotesize{$v_1\!:$}] (1) at (2, 3) {$\odot$};
% 		\draw[dashed] (1) to[out=-135,in=90] (4);
% 		\draw (1) to[out=-45,in=120] (2);
% 		\draw[dashed] (2) to[out=-135,in=45] (3);
% 		\draw[dashed] (3) to[out=-135,in=45] (4);
% 		\draw (3) to[out=-45,in=135] (5);
		
% 		\node at (2, -0.7) {(a)}; 


% 	\end{tikzpicture}
% 	\caption{(a) An example of a \dsabbr with output alphabet $\{x, y\}$. 
% 	% (b) Gadget for $\prod(\cD,v_1,v_2, k)$. (c) Gadget for $\union(\cD,v_3,v_4)$. We use dashed and solid edges for the left and right mappings, respectively. Node names are in grey at the left of each node. In (b) and (c), square nodes are the input and output nodes of each~operation.
% 	}
% 	\label{fig:gadgets}
% 	\vspace{-3mm}
% \end{figure}

\begin{figure}[t]
	\centering
	\begin{tikzpicture}[every label/.style={black!60}, ->,>=stealth',roundnode/.style={circle,inner sep=2pt},squarednode/.style={rectangle,inner sep=2pt}]
		\node [roundnode, label=180:$v_4\!:$] (4) at (0, 0) {$x$};
		\node [roundnode, label=180:$v_5\!:$] (5) at (4, 0) {$y$};
		\node [squarednode, label=180:$v_3\!:$] (3) at (2, 1) {$\cup$};
		\node [squarednode, label=180:$v_2\!:$] (2) at (3, 2) {$+2\ $};
		\node [squarednode, label=180:$v_1\!:$] (1) at (2, 3) {$\odot$};
		\draw[dashed] (1) to[out=-135,in=90] (4);
		\draw (1) to[out=-45,in=120] (2);
		\draw[dashed] (2) to[out=-135,in=45] (3);
		\draw[dashed] (3) to[out=-135,in=45] (4);
		\draw (3) to[out=-45,in=135] (5);
	\end{tikzpicture}
	\caption{An example of an \dsabbr with output alphabet $\{x, y\}$. We use dashed and solid edges for the left  and right partial function, respectively. This figure corresponds to the \dsabbr in Example~\ref{exa:fig}}
	\label{fig-ecsex}
\end{figure}


\paragraph{The enumeration algorithm} Given that every node of a \dsabbr represents a set of strings, we are interested in enumerating them with output-linear delay. Specifically, we focus on the following problem. Let $\mathcal{C}$ be a class of \dsnamesbigcaps{}.

%\vspace{0.2em}

\begin{center}
	\framebox{
		\begin{tabular}{rl}
			\textbf{Problem:} & $\enumecs[\mathcal{C}]$\\
			\textbf{Input:} & a \dsabbr $\cD \in \mathcal{C}$ and a node $v$ of $\cD$ \\
			\textbf{Output:} & Enumerate $\sem{\cD}(v)$.
		\end{tabular}
	}
\end{center}

The plan then is to provide an enumeration algorithm with output-linear delay for $\enumecs[\mathcal{C}]$ and some helpful class $\mathcal{C}$.
A reasonable strategy to enumerate the set $\sem{\cD}(v)$ is to do a traversal on the structure while accumulating the shift values in the path to each leaf. However, to be able to do this without repetitions and output-linear delay, we need to guarantee two conditions: first, that one can obtain every output from $\cD$ in only one way and, second, union and shift nodes are \emph{close} to an output node,
%(i.e., a bottom node or a product node), 
in the sense that we can always reach them in a bounded number of steps. To ensure that these conditions hold, we impose two restrictions on an ECS. 

\begin{enumerate}
	\item[(i)] We say that $\D$ is \textdef{duplicate-free} if $\D$ satisfies the following two properties: (1) for every union node $v$ it holds that $\sem{\D}(\ell(v))$ and $\sem{\D}(r(v))$ are disjoint, and (2) for every product node $v$ and for every $w \in \sem{\D}(v)$, there exists a unique way to decompose $w = w_1 \cdot w_2$ such that $w_1 \in \sem{\D}(\ell(v))$ and $w_2 \in \sem{\D}(r(v))$. Intuitively, this condition is what ensures the enumeration can be done with no repeats.
	
	\item[(ii)] We define the notion of \emph{$k$-bounded}~\dsabbr{} as follows. 
	Given an \dsabbr{} $\D$, define the \textdef{(left) output-depth} of a node $v\in V$, denoted by $\odepth_{\D}(v)$, recursively as follows:
	$\odepth_{\D}(v) = 0$ whenever $\lambda(v)\in\infAlph$ or $\lambda(v) = \odot$ (i.e., $v$ is an output node), and $\odepth_{\D}(v) = \odepth_{\D}(\ell(v))+1$ whenever $\lambda(v) \in \{\cup\}\cup\int$.
	Then, for $k\in\nat$ we say that $\D$ is $k$-bounded if $\odepth_{\D}(v)\leq k$ for all $v\in V$. Intuitively, we only limit the distance to the first output node we see to the left. Since this condition holds for every node, this is enough to ensure that in the enumeration phase the next output $o$ can always be retrieved in $|o|$ time.
\end{enumerate}


%For the first restriction, we say that an ECS $\cD$ is \emph{duplicate-free} if the following hold: (1) for every union node $v$ in $\cD$ it holds that $\sem{\cD}(\lch(v))$ and $\sem{\cD}(\rch(v))$ are disjoint and (2) for every product node $v$ and for every $w \in \sem{\cD}(v)$, there exists a unique way to decompose $w = w_1 \cdot w_2$ such that $w_1 \in \sem{\cD}(\lch(v))$ and $w_2 \in \sem{\cD}(\rch(v))$.
%
%For the second restriction, we define \emph{$k$-bounded}~\dsabbr{}. 
%Given a \dsabbr{} $\cD$, define the (left) output-depth of a node $v\in V$, denoted by $\odepth_{\cD}(v)$, recursively as follows:
%$\odepth_{\cD}(v) = 0$ whenever $\lambda(v)\in \{\odot\}\cup\Omega$, and $\odepth_{\cD}(v) = \odepth_{\cD}(\lch(v))+1$ whenever $\lambda(v) \in \{\cup\}\cup\int$.
%Then, for $k\in\nat$ we say that $\cD$ is $k$-bounded if $\odepth_{\cD}(v)\leq k$ for all $v\in V$.

\begin{prop}\label{prop:lindelay}
	Fix $k\in\nat$. Let $\mathcal{C}_k$ be the class of all  duplicate-free and $k$-bounded \dsabbrs{}. Then one can solve the problem $\enumecs[\mathcal{C}_k]$ with output-linear delay and constant preprocessing time (or equivalently, without preprocessing).
\end{prop}
\begin{proof}
	\newcommand{\len}{\mathsf{len}}
	
	Let $\D = (\infAlph, V, \ell, r, \lambda)$ be a duplicate-free and $k$-bounded \dsabbr{}.
	The algorithm that we present is a depth-first traversal of the DAG, done in a recursive fashion to ensure that after retrieving some output $w$, the next one $w'$ can be printed in $O(k\cdot (|w| + |w'|))$ time. The entire procedure is detailed in Algorithm~\ref{alg:enumeration}.
	
	\input{../algorithms/enumalg-cris}
	
	To simplify the presentation of the algorithm, we use an \emph{iterator interface} that, given a node $v$, contains all information and methods to enumerate the outputs $\sem{\D}(v)$. Specifically, an iterator $\uit$ must implement the following three methods:
	\[
	\begin{array}{rclrclrcl}
		\textsc{create}(v) & \!\!\!\!\rightarrow\!\!\!\! & \uit   \ \ \ \ \ \	 & \uit.\textsc{next} & \!\!\!\! \rightarrow \!\!\!\! & b  \ \ \ \ \ \ \ &  \uit.\textsc{print}(s)  & \!\!\!\!\rightarrow\!\!\!\! & \emptyset
	\end{array}
	\]
	where $v$ is a node, $b$ is either {\bf true} or {\bf false}, and $\emptyset$ means that the method does not return an output. 
	The first method, \textsc{create}, receives a node $v$ and creates an iterator $\uit$ of the type of $v$. We will implement three types of iterators, one for bottom nodes ($\uit_\infAlph$), one for product nodes ($\uit_\odot$), and one for union and $\int$-nodes together ($\uit_{\cup/\int}$). The second method, $\uit.\textsc{next}$, moves the iterator to the next output, returning {\bf true} if, and only if, there is an output to print. Then the last method, $\uit.\textsc{print}$, receives an integer value $s$, and writes the current output pointed by $\uit$ to the output registers after shifting the output by $s$. 
	We assume that, after creating an iterator $\uit$, one must first call $\uit.\textsc{next}$ to move to the first output before printing. Furthermore, if $\uit.\textsc{next}$ outputs {\bf false}, then the behavior of $\uit.\textsc{print}$ is undefined. Note that one can call $\uit.\textsc{print}$ several times, without calling $\uit.\textsc{next}$, and the iterator will write the same output each time in the output registers. 
	
	Assume we can implement the iterator interface for each type. Then the procedure $\textsc{Enumerate}(v)$ in Algorithm~\ref{alg:enumeration} (lines \ref{alg1enum1}-\ref{alg1enum3}) shows how to enumerate the set $\sem{\D}(v)$ by using an iterator $\uit$ for $v$. In the following, we show how to implement the iterator interface for each type and how the size of the next output bounds the delay between two outputs.
	
	
	We start by presenting the iterator $\uit_\infAlph$ for a bottom node $v$ (lines \ref{alg1bottom0}-\ref{alg1bottom11}), called a \emph{bottom node iterator}. We assume that each $\uit_\infAlph$ has internally two values, denoted by $\bnodelabel$ and $\hasnext$, where $\bnodelabel$ is a reference to $v$ and $\hasnext$ is a boolean variable. The purpose of a bottom node iterator is only to print $(\lambda(u), 1+s)$ for some shift $s$. For this goal, when we create $\uit_\infAlph$, we initialize $u$ equal to $v$ and $\hasnext = \textbf{true}$ (lines \ref{alg1bottom2}-\ref{alg1bottom3}). Then, when we call $\uit_\infAlph.\textsc{next}$ for the first time, we swap $\hasnext$ from {\bf true} to {\bf false} and output {\bf true} (i.e., there is one output ready to be returned). Then any following call to $\uit_\infAlph.\textsc{next}$ will be false (lines \ref{alg1bottom4}-\ref{alg1bottom8}). Finally, the $\uit_\infAlph.\textsc{print}$ writes the pair $(\lambda(u),1+s)$ to the output registers (lines \ref{alg1bottom9}-\ref{alg1bottom11}). Here, we assume the existence of a method {\bf print} on the RAM model for writing the next entry to the output~registers. 
	
	
	For a product node, we present a \emph{product node iterator} $\uit_\odot$ in Algorithm~\ref{alg:enumeration} (lines \ref{alg1prod0}-\ref{alg1prodlast}). 
	This iterator receives a product node $v$ with $\lambda(v) = \odot$ and stores a reference of $v$, called $u$, and two iterators $\leftit$ and $\rightit$, for iterating through the left and right node, $\ell(u)$ and $r(u)$, respectively. 
	The \textsc{create} method initializes $u$ with $v$, creates the iterators $\leftit$ and $\rightit$, and calls $\leftit.\textsc{next}$ to be prepared for the first call of $\uit_\odot.\textsc{next}$ (lines \ref{alg1prod1}-\ref{alg1prod5}).
	The purpose of $\uit_\odot.\textsc{next}$ is to fix one output for the left node $\ell(u)$ and iterate over all outputs of $r(u)$ (lines \ref{alg1prod6}-\ref{alg1prod12}). When we stop enumerating all outputs of $\sem{\D}(r(u))$, we move to the next output of $\leftit$, and iterate again over all $\sem{\D}(r(u))$ (lines \ref{alg1prod8}-\ref{alg1prod11}).
	For printing, we recursively call first the printing method of $\leftit$, and then the one of $\rightit$ (lines \ref{alg1prod13}-\ref{alg1prodlast}).
		
	The most involved case is the \emph{union/$\int$ node iterator} $\uit_{\cup/\int}$ (lines \ref{alg1union0}-\ref{alg1unionlast}). 
	This iterator receives a node $v$ of one of two types, either a union node, or a $\int$-node. It keeps a \emph{stack} $\ustack$ and an iterator~$\uit$. The elements in the stack are pairs $(u, s)$ where $u$ is a node and $s$ is an integer. We assume the standard implementation of a stack with the native methods $\text{\sf push}$, $\text{\sf pop}$, $\text{\sf top}$, and $\text{\sf depth}$: the first three define the standard operations over stacks, and $\text{\sf depth}$ counts the elements in a stack. 
	The purpose of the stack is to perform a \emph{depth-first-search} traversal of all union and $\int$ nodes below $v$, reaching all possible output nodes $u$ such that there is a path of only union and $\int$ nodes between $v$ and $u$. At every point, if an element $(u,s)$ is in the stack, then $s$ is equal to the sum of all $\int$ nodes in the path from $v$ to $u$. If the top node of $\ustack$ is a pair $(u, s)$ such that $u$ is an output node, then $\uit$ is an iterator for $u$, which enumerates all their outputs. If $p = (u,s)$, we will use the notation $p.u$ to refer to $u$.
	
	In order to perform the \emph{depth-first-search} traversal of union and $\int$ nodes, we use the auxiliary method $\textsc{traverse}(\ustack)$ (lines \ref{alg1traverse0}-\ref{alg1unionlast}). While the node $u$ at the top of $\ustack$ is a union or a shift node, we pop the top pair $(u,s)$ from $\ustack$. If $u$ is a shift node (lines~\ref{alg1traverseIfStart}-\ref{alg1traverseIfEnd}), we push the pair $(v, s')$ in the stack where $v$ is the node $\ell(u)$ pointed by $u$ and $s'$ is the sum of the current shift $s$ with the shift $\lambda(u)$.
	Otherwise, if $u$ is a union node (lines~\ref{alg1traverseElseStart}-\ref{alg1traverseElseEnd}), we first push the right pair $(r(u), s)$ followed by the left pair $(\ell(u), s)$ into the stack. 	
	The while-loop will eventually reach an output node at the top of the stack and end. 
	It is important to note that $\textsc{traverse}(\ustack)$ takes $\cO(k)$ steps, given that the ECS is $k$-bounded. Then if $k$ is fixed, the  $\textsc{traverse}$ procedure takes constant time. In Figure~\ref{fig-enum-stacks}, we illustrate the evolution of a stack $\ustack$ inside a union node iterator when we call $\textsc{traverse}(\ustack)$ several times. 
	\begin{figure}[t]
		\centering
		\input{../figures/enumfignew.tex}
		\caption{Evolution of the stack $\ustack$ (written on the bottom and represented by dashed arrows) for an iterator over the node $v$ in the figure. 
		The underlying ECS is made of union nodes, two $\int$ nodes, and six bottom nodes. The first figure is $\ustack$ after calling $\ustack \gets {\sf push}(\ustack, (v,0))$, the second is after calling $\ustack \gets\textsc{Traverse}(\ustack)$. The last two figures represent successive calls to ${\sf pop}(\ustack), \ustack \gets\textsc{Traverse}(\ustack)$.}
		% \cristian{TODO: actualizar la figura y leyenda según la nueva versión del traverse.}
		\label{fig-enum-stacks}
	\end{figure}
	
	The methods of a union/$\int$ node iterator $\uit_{\cup/\int}$ are then straightforward. For \textsc{create} (lines \ref{alg1union1}-\ref{alg1union6}), we push $(v,0)$ and then traverse $\ustack$, finding the first leftmost output node from~$v$~(lines~\ref{alg1union4}-\ref{alg1union5}). 
	Then we build the iterator $\uit$ of this output node for being ready to start enumerating their outputs (line~\ref{alg1union6}). 
	For \textsc{next}, we consume all outputs by calling $\uit.\textsc{next}$ (line~\ref{alg1unionnext1}). When there are no more outputs, we pop the top node from $\ustack$ and check if the stack is empty or not (lines~\ref{alg1unionnext2}-\ref{alg1unionnext3}). If this is the case, there are no more outputs and we output {\bf false}. Otherwise, if $\ustack$ is non-empty but the top pair $(u,s)$ of $\ustack$ contains a union node, then we apply the \textsc{traverse} method for finding the leftmost output node from~$u$~(lines \ref{alg1unionnext5}-\ref{alg1unionnext6}). When the procedure is done, we know that the node in the top pair is an output node, and then we create an iterator and move to its first output (lines~\ref{alg1unionnext7}-\ref{alg1unionnext8}). 
	For $\textsc{print}(s)$, we see the pair $(u, s')$ at the top, where we remind that $s'$ represents the sum of all $\int$ nodes on the way to $u$ (line~\ref{alg1unionprint1}), and $u$ is assumed to be an output node. Then, we call the print method of $\uit$ which is ready to write the current output, and over which we add the value $s+s'$ (line~\ref{alg1unionprint2}). 
		
	In order to prove the correctness of the enumeration procedure, one can verify that $\textsc{Enumerate}(v)$ in Algorithm~\ref{alg:enumeration} enumerates all the outputs in the set $\sem{\D}(v)$ one by one, and without repetitions, which follows from the fact that $\D$ is duplicate-free. To bound the delay between outputs, the fact that $\D$ is $k$-bounded implies that the delay is bounded by $\cO(k\cdot |w_0|)$ if $w_0$ is the first output, or $O(k\cdot (|w| + |w'|))$ if $w$ and $w'$ are the previous and next output, respectively. \edit{More precisely, we note that every iterator $\tau$ defines a {\em current} output $w_{\sf curr}$: the string that is printed when calling $\tau.{\textsc{print}}(s)$; and a {\em next} output $w_{\sf next}$: the string that is printed when calling first $\tau.\textsc{next}$ and then $\tau.\textsc{print}$; which give us following runtime bounds:}
	\begin{itemize}
		\item $\textsc{create}(v)$ takes time $\cO(k\cdot |w_0|)$, where $w_0$ is the first output in $\sem{\D}(v)$,
		\item $\textsc{next}$ takes time $\cO(k\cdot |w_0|)$ for the first call, and \edit{$\cO(k\cdot (|w_{\sf curr}|+|w_{\sf next}|))$} on each subsequent call,
		\item $\textsc{print}(s)$ takes time $\cO(k\cdot |w_{\sf curr}|)$.
	\end{itemize}
	Overall, $\textsc{Enumerate}(v)$ in Algorithm~\ref{alg:enumeration} requires $O(k\cdot (|w| + |w'|))$ delay to write the next output $w'$ in the output register, after printing the previous output $w$. 
	
	We end by pointing out that the existence of an enumeration algorithm $\enumE$ with delay $O(k\cdot (|w| + |w'|))$ between any consecutive outputs $w$ and $w'$, implies the existence of an enumeration algorithm $\enumE'$ with output-linear delay as defined in Section~\ref{sec:setting}. We start noting that $k$ is a fixed value and then the delay of $\enumE$ only depends on $|w| + |w'|$. For depending only on the next output $w'$, one can perform the following strategy for $\enumE'$: start by running~$\enumE$, enumerate the first output $w_0$, advance $k \cdot |w_0|$ more steps of $\enumE$, and stop. Then continue running $\enumE$, enumerate the next output $w_1$, advance $k \cdot |w_1|$ more steps, and stop\footnote{If advancing $k \cdot |w_1|$ more steps requires printing part of the next outputs $w_2, w_3, \ldots$, we could store these outputs in some temporary registers of the RAM model to retrieve them later.}. By repeating this enumeration process, one can verify that the delay between the $i$-th output $w_i$ and the $(i+1)$-th output $w_{i+1}$ is $O(|w_{i+1}|)$. Therefore, $\enumE'$ has output-linear delay. 
\end{proof}

\paragraph{Operations} The next step is to provide a set of operations that allow extending a \dsabbr{} $\cD$ in a way that maintains $k$-boundedness. Fix a \dsabbr{} $\cD = (\infAlph, V, \lch, \rch, \lambda)$. Then for any $\oout \in \infAlph$, $v_1, \ldots, v_4, v \in V$ and $k\in\int$, we define these four operations, given alongside their expected semantics:
%\[
%\begin{array}{rclrclrcl}
%	\add(\oout) \! \! \! &\to&\! \! \! v'  \ \ \ \ \ \  \prod(v_1, v_2) \! \! \! &\to&\! \! \! v'   \\  \union(v_3, v_4) \! \! \! &\to&\! \! \! v' \ \ \ \ \ \  \shiftop(v, k) \! \! \! \! \! &\to&\! \! \! v'
%\end{array}
%\]
\[
\edit{\begin{array}{rl}
	\add(\oout) \ \to\  v'  \ \ \ \ \ \  &\sem{\cD}(v') := \{(\oout,1)\}\\
	\prod(v_1, v_2) \ \to\ v' \ \ \ \ \ \  &\sem{\cD}(v') := \sem{\cD}(v_1) \cdot \sem{\cD}(v_2) \\  
	\union(v_3, v_4) \ \to\  v' \ \ \ \ \ \ &\sem{\cD}(v') := \sem{\cD}(v_3) \cup \sem{\cD}(v_4)\\
	\shiftop(v, k) \ \to\ v' \ \ \ \ \ \ &\sem{\cD}(v') := \shift(\sem{\cD}(v), k)
\end{array}}
\]
Here we assume that the $\union$ and $\prod$ are called only when properties (1) and (2) of a duplicate-free \dsabbr{} hold, namely, $\sem{\cD}(v_3)$ and $\sem{\cD}(v_4)$ are disjoint; and, for every $w \in \sem{\cD}(v_1) \cdot \sem{\cD}(v_2)$, there exists a unique way to decompose $w = w_1 \cdot w_2$ such that $w_1 \in \sem{\cD}(v_1)$ and $w_2 \in \sem{\cD}(v_2)$.

Strictly speaking, each operation above should receive as input the data structure $\cD$, and output a fresh node $v'$ plus a new data structure $\cD' = (\infAlph, V', \lch', \rch', \lambda')$ such that $\cD'$ is an extension of $\cD$, namely, $\mathsf{obj} \subseteq \mathsf{obj}'$ for every $\mathsf{obj} \in \{V, \lch, \rch, \lambda\}$ and $v' \in V' \setminus V$. Note that we assume that each operation would only extend the data structure with new nodes and that old nodes are immutable after each operation. By this, we mean that once a node $v$ is created, and the values $\ell(v)$, $r(v)$ and $\lambda(v)$ assigned, none of these values ever change again. This also implies that the entire subgraph that is reachable from $v$, and thus, the set $\sem{\cD}(v)$, also stay the same. For simplification, we will not explicitly refer to $\cD$ on the operations above, although they modify $\cD$ directly by adding new nodes. 

To define the above operations, we impose further restrictions on the structure below the operations' input nodes to ensure $k$-boundedness. Towards this goal, we introduce the notion of \textdef{safe nodes}.

We say that a node $v \in V$ is \emph{safe} if it is a shift node over an output node, or over a union node with an output node on the left and a shift node with output depth of at most 2 on the right. \edit{More precisely, $v$ is safe iff $\lambda(v) \in \mathbb{Z}$, and either: $\lch(v)$ is an output node; or $\lch(v)$ is a union node with $\odepth_{\cD}(\lch(v)) = 1$ and $\rch(\lch(v))$ is a shift node with $\odepth_{\cD}(\rch(\lch(v))) \leq 2$. }
In other words, $v$ is safe if 
The next step is to show that all operations over \dsabbrs{} receive only safe nodes and output only safe nodes. 
As we will see, safeness will be a light structural restriction on the operations' input nodes that is enough to maintain $k$-boundedness after each operation.  

Next, we show how to implement each operation assuming that every input node is safe. In fact, the cases of $\add$ and $\shiftop$ are straightforward. 
For $\add(\oout)\to v'$ we extend $\cD$ with two fresh nodes $v'$ and $u$ such that $\lambda(u) = \oout$, $\lambda(v') = 0$, and $\lch(v') = u$. In other words, we hang a fresh $0$-shift node $v'$ over a fresh $\oout$-node $u$, and output $v'$. 
For $\shiftop(v, k) \to v'$, add the fresh node $v'$ to $\cD$, and set $\ell(v') = \ell(v)$ and $\lambda(v') = \lambda(v) + k$.
One can easily check that in both cases the node $v'$ represents the desired set, is safe, and $k$-boundedness is preserved.

To show how to implement $\prod(v_1, v_2)\to v'$, recall that $v_1$ and $v_2$ are safe and, in particular, both are shift nodes. 
Then we need to extend $\cD$ with fresh nodes $v'$, $v''$, and $v'''$ such that  $\ell(v') = v''$, $\ell(v'') = \ell(v_1)$, $r(v'') = v'''$, $\ell(v''') = \ell(v_2)$, $\lambda(v') = \lambda(v_1)$, $\lambda(v'') = \odot$ and $\lambda(v''') = \lambda(v_2) - \lambda(v_1)$. 
Figure~\ref{fig:gadgets}(a) shows a diagram of this gadget. One can easily check that $v'$ represents the product of $v_1$ and $v_2$, $v'$ is safe, and the new version of $\cD$ is $k$-bounded whenever $\cD$ is also $k$-bounded.

The last operation is $\union(v_3, v_4)\to v'$. The strategy is then to prove that if $v_3$ and $v_4$ are safe nodes, then we can implement the operator and produce a safe node $v'$. Let us define $v'$ as follows:
\begin{itemize}
	\item If at least one among $\ell(v_3)$ and $\ell(v_4)$ is an output node, assume without loss of generality that it is $\ell(v_3)$. We extend $\cD$ with nodes $v'$, $v''$ and $v'''$, where $\ell(v') = v''$, $\ell(v'') = \ell(v_3)$, $r(v'') = v'''$, $\ell(v''') = \ell(v_4)$, $\lambda(v') = \lambda(v_3)$, $\lambda(v'') = \cup$ and $\lambda(v''') = \lambda(v_4) - \lambda(v_3)$. 
	This construction is identical to the $\prod$ construction shown in Figure~\ref{fig:gadgets}(a), except replacing $v_1$ and $v_2$ by $v_3$ and $v_4$ respectively, and $\lambda(v'')$ from $\odot$ to $\cup$.
	%This construction is illustrated in FIgure~\ref{fig-theo-ds}. 
	\item When both $u_3 = \lch(v_3)$ and $u_4 = \lch(v_4)$ are union nodes, let $k'_1 = \lambda(r(u_3))$ and let $k'_2 = \lambda(r(u_4))$. 
	We extend $\cD$ with fresh nodes $v',v'_1,v'_2,v'_3,v'_4,v'_5$ and $v'_6$. 
	Define $\lambda(v') = k_1$, $\lambda(v'_1) = \cup$, $\lambda(v'_2) = k_2 - k_1$, $\lambda(v'_3) = \cup$,  $\lambda(v'_4) = k_1+k'_1-k_2$, $\lambda(v'_5) = \cup$ and $\lambda(v'_6) = k_2 + k'_2 - k_1 - k'_1$. 
	Then define $\ell(v') = v'_1$, $\ell(v'_1) = \ell(u_3)$, $r(v'_1) = v'_2$, $\ell(v'_2) = v'_3$, $\ell(v'_3) = \ell(u_4)$, $r(v'_3) = v'_4$, $\ell(v'_4) = v'_5$, $\ell(v'_5) = \ell(r(u_3))$, $r(v'_5) = v'_6$ and $\ell(v'_6) = \ell(r(u_4))$. 
	We show an illustration of this gadget in Figure~\ref{fig:gadgets}(b).
\end{itemize}

%Without loss of generality, assume that $v_3$ has an output node as its left child. 
%It can be seen that $v'$ is a safe node since the left child of $v''$ is an output node, and $v'''$ has output depth at most 2, either if $\ell(v_4)$ is an output node, or if $\ell(v_4)$ is a union node whose left child is an output node. Since $\cD$ was assumed to be 3-bounded, and this operation only adds nodes with output depth at most 2, the new version of $\cD$ is 3-bounded as well. 


%\begin{figure}
%	\centering
%	\begin{tikzpicture}[every label/.style={black!60}, ->,>=stealth',roundnode/.style={circle,inner sep=1pt},squarednode/.style={rectangle,inner sep=2pt}, scale=0.85]
	%		\node[squarednode] (0) at (0, 0) {$\ell(v_3)$};
	%		\node[squarednode, draw, label=180:\footnotesize{$v_3\!:$}] (2) at (2, 1) {$k_1$};
	%		\node[squarednode] (3) at (4, 0) {$\ell(v_4)$};
	%		\node[squarednode, draw, label=180:\footnotesize{$v_4\!:$}] (5) at (6, 1) {$k_2$};
	%		\node[squarednode, label=180:\footnotesize{$v'''\!:$}] (7) at (5.5, 1.7) {$(k_2-k_1)$};
	%		\node[squarednode, label=180:\footnotesize{$v''\!:$}] (8) at (3, 2.6) {$\cup$};
	%		\node[squarednode, draw, label=180:\footnotesize{$v'\!:$}] (9) at (4.5, 3.6) {$k_1$};
	%		\draw[dashed] (2.south west) to[out=-135,in=45] (0);
	%		\draw[dashed] (5.south west) to[out=-135,in=45] (3);
	%		\draw[dashed] (7.south west) to[out=-135,in=90] (3);
	%		\draw (8) to[out=-45,in=135] (7.north west);
	%		\draw[dashed] (8) to[out=-135,in=90] (0);
	%		\draw[dashed] (9.south west) to[out=-135,in=90] (8);
	%		
	%	\end{tikzpicture}
%	\caption{Gadget used in Theorem~\ref{theo:data-structure}.}
%	\label{fig-theo-ds}
%\end{figure}


We can prove that the last construction has several interesting properties.
First, one can check that $\sem{\cD}(v') = \sem{\cD}(v_3)\cup \sem{\cD}(v_4)$ since each shift value is 
%carefully 
constructed so that the accumulated shift value from $v'$ to each node remains unchanged.
Thus, the semantics is well-defined. 
Second, $\union$ can be computed in constant time in $|\cD|$ given that we only need to add a fixed number of fresh nodes.
%and the operation is fully-persistent given that we connect them to previous nodes without modifying $\cD$. 
Furthermore, the produced node $v'$ is safe, even though some of the new nodes are not necessarily safe. 
Finally, the new $\cD$ is 3-bounded whenever $\cD$ is 3-bounded. This is straightforward to see for the case when $\ell(v_3)$ (or $\ell(v_4)$) is an output node. To see this for the second case, we first have to notice that $\ell(u_3)$ and $\ell(u_4)$ are output nodes, and that $\odepth(\ell(r(u_3)))\leq 1$ and $\odepth(\ell(r(u_4)))\leq 1$. We can check the depth of each node going from the bottom to the top: $\odepth(v_6') \leq 2$, $\odepth(v_5') \leq 2$, $\odepth(v_4') \leq 3$, $\odepth(v_3')\leq 1$, $\odepth(v_2') \leq 2$, $\odepth(v_1') \leq 1$ and $\odepth(v')\leq 2$.

\begin{figure}[t]
	\centering
	\begin{tikzpicture}[every label/.style={black!60}, ->,>=stealth',roundnode/.style={circle,inner sep=1pt},squarednode/.style={rectangle,inner sep=2pt}, scale=0.85]
		
		% \begin{scope}[xshift=-7cm, yshift=6cm]
		% \node [roundnode, label=180:\footnotesize{$v_4\!:$}] (4) at (0, 0) {$x$};
		% \node [roundnode, label=180:\footnotesize{$v_5\!:$}] (5) at (4, 0) {$y$};
		% \node [squarednode, label=180:\footnotesize{$v_3\!:$}] (3) at (2, 1) {$\cup$};
		% \node [squarednode, label=180:\footnotesize{$v_2\!:$}] (2) at (3, 2) {$+2\ $};
		% \node [squarednode, label=180:\footnotesize{$v_1\!:$}] (1) at (2, 3) {$\odot$};
		% \draw[dashed] (1) to[out=-135,in=90] (4);
		% \draw (1) to[out=-45,in=120] (2);
		% \draw[dashed] (2) to[out=-135,in=45] (3);
		% \draw[dashed] (3) to[out=-135,in=45] (4);
		% \draw (3) to[out=-45,in=135] (5);
		
		% \node at (2, -0.7) {(a)}; 
		% \end{scope}
	
		\begin{scope}[xshift=-8cm, yshift=0cm]
			\node[squarednode] (0) at (0, 0) {$\ell(v_1)$};
			\node[squarednode, draw, label=180:\footnotesize{$v_1\!:$}] (2) at (2, 1.2) {$k_1$};
			\node[squarednode] (3) at (4, 0) {$\ell(v_2)$};
			\node[squarednode, draw, label=180:\footnotesize{$v_2\!:$}] (5) at (6, 1.2) {$k_2$};
			\node[squarednode, label=180:\footnotesize{$v'''\!:$}] (7) at (5.5, 2.1) {$(k_2-k_1)$};
			\node[squarednode, label=180:\footnotesize{$v''\!:$}] (8) at (3, 3.0) {$\odot$};
			\node[squarednode, draw, label=180:\footnotesize{$v'\!:$}] (9) at (4.5, 4.2) {$k_1$};
			\draw[dashed] (2.south west) to[out=-135,in=45] (0);
			\draw[dashed] (5.south west) to[out=-135,in=45] (3);
			\draw[dashed] (7.south west) to[out=-135,in=90] (3);
			\draw (8) to[out=-45,in=135] (7.north west);
			\draw[dashed] (8) to[out=-135,in=90] (0);
			\draw[dashed] (9.south west) to[out=-135,in=90] (8);
			
			\node at (3, -0.7) {(a)}; 
	
		\end{scope}
		
		
		\node[squarednode] (0) at (0, 0) {$\ell(u_3)$};
		\node[squarednode] (1) at (2, 0) {$\ell(r(u_3))$};
		\node[squarednode, label=180:\footnotesize{$r(u_3)\!:$}] (1p) at (2, 1) {$k_1'$};
		\node[squarednode, label=180:\footnotesize{$u_3\!:$}] (2) at (1, 2) {$\cup$};
		\node[squarednode, draw, label=180:\footnotesize{$v_3\!:$}] (2p) at (1.2, 3) {$k_1$};
		\node[squarednode] (0b) at (4, 0) {$\ell(u_4)$};
		\node[squarednode] (1b) at (6, 0) {$\ell(r(u_4))$};
		\node[squarednode, label=180:\footnotesize{$r(u_4)\!:$}] (1bp) at (6, 1) {$k_2'$};
		\node[squarednode, label=180:\footnotesize{$u_4\!:$}] (2b) at (5, 2) {$\cup$};
		\node[squarednode, draw, label=180:\footnotesize{$v_4\!:$}] (2bp) at (5.2, 3) {$k_2$};
		\node[squarednode, draw, label=180:\footnotesize{$v'\!:$}] (vp) at (3.5, 9) {$k_1$};
		\node[squarednode, label=180:\footnotesize{$v_1'\!:$}] (v) at (3, 8) {$\cup$};
		\node[squarednode, label=180:\footnotesize{$v_2'\!:$}] (u1p) at (4.5, 7) {$k_2 - k_1$};
		\node[squarednode, label=180:\footnotesize{$v_3'\!:$}] (u1) at (4, 6) {$\cup$};
		\node[squarednode, label=180:\footnotesize{$v_4'\!:$}] (u2p) at (5.5, 5) {$k_1+k_1'-k_2$};
		\node[squarednode, label=180:\footnotesize{$v_5'\!:$}] (u2) at (4.8, 4) {$\cup$};
		\node[squarednode, label=180:\footnotesize{$v_6'\!:\!\!\!\!\!\!\!$}] (u3) at (7, 3) {$
			\begin{array}{r}
			k_2 +k_2' \\
			- k_1 - k_1'
			\end{array}$};
		\draw[dashed] (vp) to (v);
		\draw[dashed] (v) to[out=-135, in=110] (0);
		\draw (v) to[out=-45] (u1p);
		\draw[dashed] (u1p) to (u1);
		\draw[dashed] (u1) to[out=-135, in=110] (0b);
		\draw (u1) to[out=-45] (u2p);
		\draw[dashed] (u2p) to (u2);
		\draw[dashed] (u2) to[out=-135, in=45] (1);
		\draw (u2) to[out=-45] (u3);
		\draw[dashed] (u3) to[out=-135,in=45] (1b);
		\draw[dashed] (2) to[out=-135, in=90] (0);
		\draw (2) to[out=-45,in=135] (1p);
		\draw[dashed] (1p) to[out=-135,in=90] (1);
		\draw[dashed] (2p) to (2);
		\draw[dashed] (2b) to[out=-135, in=90] (0b);
		\draw (2b) to[out=-45,in=135] (1bp);
		\draw[dashed] (1bp) to[out=-135,in=90] (1b);
		\draw[dashed] (2bp) to (2b);
		
		\node at (3, -0.7) {(b)}; 
	\end{tikzpicture}
	\caption{
	(a) Gadget for $\prod(\cD,v_1,v_2, k)$. 
	(b) Gadget for $\union(\cD,v_3,v_4)$. 
	We use dashed and solid edges for the left and right child, respectively. 
	Node names are in grey at the left of each node. Nodes in square boxes are the input and output nodes of each~operation.}
	\label{fig:gadgets}
%	 \vspace{-3mm}
\end{figure}

By the previous discussion, if we start with a \dsabbr\ $\cD$ which is 3-bounded (in particular, empty) and we apply the $\add$, $\prod$, $\union$ and $\shiftop$ operators between safe nodes (which also produce safe nodes), then the result is 3-bounded as well.
Furthermore, the data structure is fully-persistent~\cite{DriscollSST86}: for every node $v$ in $\cD$, $\sem{\cD}(v)$ is immutable after each operation. Finally, by Proposition~\ref{prop:lindelay}, the result can be enumerated with output-linear~delay.

\begin{thm}\label{theo:data-structure}
	The operations $\add$, $\prod$, $\union$ and $\shiftop$ take constant time and are fully persistent. Furthermore, if we start from an empty \dsabbr\ $\cD$ and apply these operations over safe nodes, the result node $v'$ is always a safe node and the set $\sem{\cD}(v)$ can be enumerated with output-linear delay (without preprocessing) for every node $v$.
\end{thm} 



%From here onwards, we require any ECS to have the additional property that shift nodes can only be child of another node if, and only if, they are the right child. We call this the {\em shifts-on-the-right} property. In particular, it requires that no shift node is a child of another shift node. The following lemma shows that requiring this does not restrict the language described by the structure, and that the size blowup is minimal.
%
%\begin{lemma}
%	For a given $k$-bounded ECS $\cD$ with node set $V$, there exists a $k$-bounded shifts-on-the-right compliant ECS $\cD'$ with node set $V'$ and a mapping function $\beta:V\to V'$ such that for every node $v\in V$, they satisfy $\sem{\cD}(v) = \sem{\cD'}(\beta(v))$. Furthermore, $|V'| \leq 3\cdot|V|$ and $\cD'$ is duplicate-free if $\cD$ is duplicate-free.
%\end{lemma}
%\begin{proof}[Proof sketch.]
%	The construction is done recursively by mapping each node $u$ in $\cD$ to a shift node in $\cD'$ with a non-shift child. Eventually, each of these shift nodes has a value equal to the accumulated values of the shift nodes in the longest path of left-children that starts in $u$, and this makes it unnecessary to have any shift node as a left child. This essentially pushes the shift values upwards, which means that in product and union nodes the right child are also affected. This is solved by counterweighting the value of the shift node that the right child is mapped to.
%\end{proof}
%Next, we show how to implement each operation. In fact, the case of $\add$ is straightforward. 
%For $\add(\cD,a)\to(\cD',v')$ define $V' := V \cup \{v'\}$, $I' := I$, $\lambda'(v') = a$. 
%One can easily check that $\L_{\cD'}(v') = \{a\}$ as expected. 
%To show how to implement $\prod(\cD,v_1, v_2)\to(\cD',v') $ suppose w.l.o.g. that $v_1$ and $v_2$ are shift nodes -- if some $v_i$ is not a shift node we can replace it by a shift node $u$ with label $\lambda(u) = 0$ and $\ell(u) = v_i$. Define $V' = V\cup \{v',v'',v'''\}$, $I' = I\cup\{v',v'',v'''\}$, $\ell(v') = v''$, $\ell(v'') = \ell(v_1)$, $r(v'') = v'''$, $\ell(v''') = \ell(v_2)$, $\lambda(v') = \lambda(v_1)$, $\lambda(v'') = \odot$ and $\lambda(v''') = \lambda(v_2) - \lambda(v_1)$. See Figure~\ref{fig-prod-def}.
%
%\begin{figure}[h]
%	\centering
%	\begin{tikzpicture}[->,>=stealth',roundnode/.style={circle,inner sep=1pt},squarednode/.style={rectangle,inner sep=2pt}, scale=0.95]
%		\node[squarednode] (0) at (0, 0) {$\ell(v_1)$};
%		\node[squarednode] (2) at (2, 1) {$v_1$\scriptsize{$[+x]$}};
%		\node[squarednode] (3) at (4, 0) {$\ell(v_2)$};
%		\node[squarednode] (5) at (6, 1) {$v_2$\,\scriptsize{$[+y]$}};
%		\node[squarednode] (7) at (5.5, 1.7) {$v'''$\scriptsize{$[+k+y  - x]$}};
%		\node[squarednode] (8) at (3, 2.6) {$\ v''$\scriptsize{$[\odot]$}};
%		\node[squarednode] (9) at (4.5, 3.6) {$v'$\scriptsize{$[+x]$}};
%		\draw[dashed] (2.south west) to[out=-135,in=45] (0);
%		\draw[dashed] (5.south west) to[out=-135,in=45] (3);
%		\draw[dashed] (7.south west) to[out=-135,in=90] (3);
%		\draw (8) to[out=-45,in=135] (7.north west);
%		\draw[dashed] (8) to[out=-135,in=90] (0);
%		\draw[dashed] (9.south west) to[out=-135,in=90] (8);
%	\end{tikzpicture}
%	\caption{Gadget for $\prod(\cD,v_1,v_2, k)$. Dashed and solid lines denote the mappings in $\ell'$ and $r'$ respectively.}
%	\label{fig-prod-def}
%	\vspace{-3mm}
%\end{figure}
%
%%\cristian{Aquí falta decir los casos cuando el $v_1$ no es un shift. También deberías discutir brevemente porque el resultado es $k$-bounded.}
%
%To define the union, we need to be a bit more careful to ensure $k$-boundedness. Towards this goal, we introduce the notion of {\em safe} nodes.
%For a non-shift node $v\in V$, we say that $v$ is safe if (1) $\odepth_{\cD}(v) \leq 1$, and (2) if $\odepth_{\cD}(v) = 1$, thus, if $r(v)$ is not a shift node, then $\odepth_{\cD}(r(v)) \leq 1$, and if it is, then $\odepth_{\cD}(\ell(r(v))) \leq 1$. If $v$ is a shift node, we say that it is safe if its left child is safe. In other words, $v$ is safe if (i) $v$ is an output node, or (ii) its left child is an output node, and the right child is either an output node, has output depth 1, or is a shift node with a left child like one of these two, or (iii) is a shift node with a left child that either satisfies (i) or (ii).
%Note that, by definition, a leaf or a product node, or a shift node that is a parent thereof, are safe nodes and, thus, the $\add$ and $\prod$ operations always produce safe nodes. The trick then is to show that, if $v_3$ and $v_4$ are safe nodes, then we can implement $\union(\cD,v_3, v_4)\to (\cD',v')$ and produce a safe node $v'$. For the sake of presentation, we only provide the construction for the most involved case, which is when $v_3$ and $v_4$ are shift nodes with safe left children that satisfy (2).
%
%
%
%%\begin{itemize}
%%	\item  If $v_3$ or $v_4$ are output nodes then $V' := V\cup\{v'\}$, $I' := I\cup\{v'\}$, and $\lambda(v') := \cup$. Moreover, if $v_3$ is the output node, then $\ell'(v') := v_3$ and $r'(v') := v_4$. Otherwise, we connect $\ell'(v') := v_4$ and~$r'(v') := v_3$.
%%	\item If $v_3$ and $v_4$ are not output nodes (i.e. both are union nodes), then $V' := V \cup\{v',u_1,u_2\}$, $I' := I\cup\{v',u_1,u_2\}$, $\ell'(v') := \ell(v_3)$, $r'(v') := u_1$, and $\lambda'(v') := \cup$; $\ell'(u_1) := \ell(v_4)$, $r'(u_1) := u_2$, and $\lambda'(u_1) := \cup$; $\ell'(u_2) := r(v_3)$, $r'(u_2) := r(v_4)$, and $\lambda'(u_2) := \cup$.
%%\end{itemize}
%This gadget is depicted in Figure~\ref{fig-union-def}.
%Interestingly, this construction has several properties.
%First, one can check that $\L_{\cD'}(v') = \sem{\cD}(v_3)\cup \sem{\cD}(v_4)$ since each shift value is carefully constructed so that the accumulated shift value from $v'$ to each node unchanged.
%Thus, the semantics is well-defined. 
%Second, $\union$ can be computed in constant time in $|\cD|$ given that we only need to add a fixed number of fresh nodes.
%%and the operation is fully-persistent given that we connect them to previous nodes without modifying $\cD$. 
%Furthermore, the produced node $v'$ is safe in $\cD'$, although some of the new nodes are not necessarily safe. 
%Finally, $\cD'$ is 3-bounded whenever $\cD$ is 3-bounded. To see this, we first have to notice that $\ell(\ell(v_3))$ and $\ell(\ell(v_4))$ are output nodes, and that $\odepth_{\cD'}(\ell(v_3'))\leq 1$ and $\odepth_{\cD'}(\ell(v_4')) \leq 1$. We can check the depth of each node going from the bottom to the top: $\odepth(u_3) \leq 2$, $\odepth(u_2') \leq 2$, $\odepth(u_2) \leq 3$, $\odepth(u_1')\leq 1$, $\odepth(u_1) \leq 2$, $\odepth(v'') \leq 1$ and $\odepth(v')\leq 2$.
%
%Lastly, we show how to implement $\shiftop(\cD, v_5, s) \to (\cD', v')$. Simply define $V' = V\cup\{v'\}$, $I' = I \cup \{v'\}$, and if $v_5$ is not a shift node, set $\ell(v') = v_5$ and $\lambda(v') = s$, otherwise set $\ell(v') = \ell(v_5)$ and $\lambda(v') = \lambda(v_5) + s$.
%
%Given that the output depths of all fresh nodes in $\cD'$ are bounded by $3$ and $\cD$ is $3$-bounded, then we conclude that $\cD'$ is $3$-bounded as well.
%
%\begin{figure}[t]
%	\centering
%	\begin{tikzpicture}[->,>=stealth',roundnode/.style={circle,inner sep=1pt},squarednode/.style={rectangle,inner sep=2pt}, scale=0.85]
%		\node[squarednode] (0) at (0, 0) {$\ell(\ell(v_3))$};
%		\node[squarednode] (1) at (2, 0) {$\ell(v_3')$};
%		\node[squarednode] (1p) at (2, 1) {$v_3'$\scriptsize{$[+x_2]$}};
%		\node[squarednode] (2) at (1, 2) {$\ \ \ \ \ell(v_3)$\scriptsize{$[\cup]$}};
%		\node[squarednode] (2p) at (1.5, 3) {$v_3$\scriptsize{$[+x_1]$}};
%		\node[squarednode] (0b) at (4, 0) {$\ell(\ell(v_4))$};
%		\node[squarednode] (1b) at (6, 0) {$\ell(v_4')$};
%		\node[squarednode] (1bp) at (6, 1) {$v_4'$\scriptsize{$[+y_2]$}};
%		\node[squarednode] (2b) at (5, 2) {$\ \ \ \ell(v_4)$\scriptsize{$[\cup]$}};
%		\node[squarednode] (2bp) at (5.5, 3) {$v_4$\scriptsize{$[+y_1]$}};
%		\node[squarednode] (vp) at (3.5, 9) {$\ \ \ \ \ v'$\scriptsize{$[+x_1]$}};
%		\node[squarednode] (v) at (3, 8) {$\ \ \ \ v''$\scriptsize{$[\cup]$}};
%		\node[squarednode] (u1p) at (4.5, 7) {$\ \ \ \ \ \ \ \ \ \ \ \ \ u_1$\scriptsize{$[+y_1 - x_1]$}};
%		\node[squarednode] (u1) at (4, 6) {$\ \ \ \ u_1'$\scriptsize{$[\cup]$}};
%		\node[squarednode] (u2p) at (5.5, 5) {$\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ u_2$\scriptsize{$[+x_1+x_2 -y_1]$}};
%		\node[squarednode] (u2) at (5, 4) {$\ \ \ u_2'$\scriptsize{$[\cup]$}};
%		\node[squarednode] (u3) at (7, 3) {$\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ u_3$\scriptsize{$[+y_1 +y_2 - x_1 - x_2]$}};
%		\draw[dashed] (vp) to (v);
%		\draw[dashed] (v) to[out=-135, in=110] (0);
%		\draw (v) to[out=-45] (u1p);
%		\draw[dashed] (u1p) to (u1);
%		\draw[dashed] (u1) to[out=-135, in=110] (0b);
%		\draw (u1) to[out=-45] (u2p);
%		\draw[dashed] (u2p) to (u2);
%		\draw[dashed] (u2) to[out=-135, in=45] (1);
%		\draw (u2) to[out=-45] (u3);
%		\draw[dashed] (u3) to[out=-135,in=45] (1b);
%		\draw[dashed] (2) to[out=-135, in=90] (0);
%		\draw (2) to[out=-45,in=135] (1p);
%		\draw[dashed] (1p) to[out=-135,in=90] (1);
%		\draw[dashed] (2p) to (2);
%		\draw[dashed] (2b) to[out=-135, in=90] (0b);
%		\draw (2b) to[out=-45,in=135] (1bp);
%		\draw[dashed] (1bp) to[out=-135,in=90] (1b);
%		\draw[dashed] (2bp) to (2b);
%	\end{tikzpicture}
%	\caption{Gadget for $\union(\cD,v_3,v_4)$. Nodes $v'$, $u_1$, $u_2$, $u_3$, $v_3$, $v_3'$, $v_4$ and $v_4'$ are shift nodes with label equal to the number between brackets. Nodes $v''$, $u_1$, $u_2$, $\ell(v_3)$ and $\ell(v_4)$ are union nodes.}
%	\label{fig-union-def}
%	\vspace{-3mm}
%\end{figure}
%%\cristian{La definición de safe dice que el nodo debe tener odepth menor o igual que 1 pero el resultado tiene odepth 2. ¿Esta bien?}
%
%By the previous discussion, if we start with an \dsabbr\ $\cD$ which is 3-bounded (or empty) and we apply the $\add$, $\prod$, $\union$ and $\shiftop$ operators between safe nodes (which also produce safe nodes), then the result is 3-bounded as well. Finally, by Proposition~\ref{ds:lindelay}, the result can be enumerated with output-linear delay.
%
%\begin{theorem}\label{theo:data-structure}
%	The operations $\add$, $\prod$, $\union$ and $\shiftop$ take constant time and are fully-persistent. Furthermore, if we start from an empty \dsabbr\ $\cD$ and apply $\add$, $\prod$, $\union$ and $\shiftop$ over safe nodes, the partial results $(\cD', v')$ satisfies that $v'$ is always a safe node and the set $\L_{\cD'}(v)$ can be enumerated with output-linear delay for every node $v$.
%\end{theorem}  

\paragraph{The empty- and $\epsilon$-nodes} The last step of constructing our model of \dsabbr{} is the inclusion of two special nodes that produce the empty set and the empty string, called empty- and $\epsilon$-node, respectively. 
%For the sake of presentation, we include both nodes here, although they are crucial for our evaluation algorithm in Section~\ref{sec:evaluation}.

We start with the \emph{empty node}, which is easier to incorporate into a \dsabbr{}. Consider a special node $\bot$ and include it on every \dsabbr{} $\cD$, such that $\sem{\cD}(\bot) = \emptyset$. 
Then extend the operations $\prod$, $\union$, and $\shiftop$ accordingly to the empty set, namely, $\prod(v_1, v_2) \to \bot$ whenever $v_1$ or $v_2$ is equal to $\bot$, $\union(v, \bot) = \union(\bot, v) \to v$, and $\shiftop(\bot, k) \to \bot$ for every nodes $v_1, v_2, v$, and $k \in \int$. It is easy to check that one can include the $\bot$-node into \dsabbrs{} without affecting the guarantees of Theorem~\ref{theo:data-structure}.

The other special node is the \emph{$\epsilon$-node}. Let $\eps$ denote a special node, included on every \dsabbr{} $\cD$, such that $\sem{\cD}(\epsilon) = \{\epsilon\}$. With these new nodes in a \dsabbr{}, we need to revise our notions of output-depth, duplicate-free, and $k$-boundedness to change the enumeration algorithm, and to extend the operations $\add$, $\prod$, $\union$, and $\shiftop$ over so-called $\epsilon$-safe nodes (i.e., the extension of safe nodes with $\epsilon$). 

%Given space restrictions, we show the use of $\epsilon$-nodes in an extended version and how we can preserve Proposition~\ref{prop:lindelay} and Theorem~\ref{theo:data-structure}. 

%	Extending these four operations to deal with empty nodes is straightforward, and this has already been defined, so we will focus on operations that deal with the $\eps$-node.
	First, we add the condition that for any \dsabbr $\cD$ the $\eps$-node is either parentless (and thus disconnected to the rest of the structure), or if it has any parents, then they must be parentless union nodes, and the $\eps$-node must be the left child of each. We call this the \textdef{$\eps$-condition}. We will see that any node that might be the result of applying the operations $\add$, $\prod$, $\union$ and $\shiftop$ is equivalent to a node in a \dsabbr $\cD$ that satisfies this. 
	
	The notions of output-depth, duplicate-free, and $k$-boundedness are mostly unchanged in this setting: If $v$ is the $\eps$-node, then $\odepth(v) = 0$, and if $v$ is a union node with the $\eps$-node as its left child, $\odepth(v) = 1$. No other node has the $\eps$-node as a descendant, so the definition of output-depth remains the same; and the definitions of duplicate-free and $k$-bounded remain unchanged as well. By assuming the $\eps$-condition, one can see that enumeration remains identical as before, except now the $\eps$-node might be seen once as the left child of the root. Then we can state the following as a corollary of Proposition~\ref{prop:lindelay}:
	
	\begin{cor}\label{prop:lindelayeps}
		Fix $k\in\nat$. Let $\mathcal{C}_k$ be the class of all  duplicate-free and $k$-bounded \dsabbrs{} that satisfy the $\eps$-condition. Then one can solve the problem $\enumecs[\mathcal{C}_k]$ with output-linear delay and without preprocessing (i.e. constant preprocessing time).
	\end{cor}
	
	
	We now define the notion of \textdef{$\eps$-safe} nodes. These are nodes $v$ which satisfy one of three conditions: (1) $v$ is the $\eps$-node, (2) $v$ is safe and none of its descendants is the $\eps$-node, and (3) $v$ is a union node, its left child is the $\eps$-node, and its right child is a safe node for which none of its descendants is the $\eps$-node. 
	To guide the constructions, we call these conditions 1, 2 and 3.
	These conditions will allow us to use the constructions already given for $\prod$, $\union$, and $\shiftop$ over safe nodes, such as node $v$, in the case of condition 2, or $r(v)$, in the case of condition 3.
	The rest of this proof will be extending these operations to work over $\eps$-safe nodes, and check that they can be done in constant time, return an $\eps$-safe node, maintain the $\eps$-condition in the \dsabbr, and satisfy the specifications of each operation (i.e., that for the resulting node $v'$ the set $\sem{\cD}(v')$ contains what it should). 
	
	We define the operation $\add$ the same as in a \dsabbr without $\eps$. The operation $\add(\eps)$ is not defined since the $\eps$-node is always part of $\cD$.
	
	The $\prod$ case is somewhat more involved. First, assume that some node among $v_1$ and $v_2$ is the $\eps$-node (condition 1). Without loss of generality, assume that $v_1 = \eps$ . If $v_2$ is the $\eps$-node as well, we simply return $v_1$; and if $v_2$ is not the $\eps$-node (conditions 2 or 3), we simply return $v_2$. The requirements of the construction follow trivially. Now, assume that both $v_1$ and $v_2$ satisfy condition 2. For this case we simply return $\prod(v_1, v_2)$ as it was defined for a \dsabbr without $\eps$. Lastly, assume at least one node among $v_1$ and $v_2$ satisfies condition~3 and none of them are the $\eps$-node. These cases are depicted in Figure~\ref{fig-prod-multi-gadget}. 
	We describe them formally as follows, assuming that $v'$ is the output and using the operations $\union$ and $\prod$ as they were defined for a \dsabbr without $\eps$.
	\begin{itemize}
		\item If $v_1$ satisfies condition 2 and $v_2$ satisfies condition 3, define $v'' \gets \prod( v_1, r(v_2))$ and $v' \gets \union( v_1, v'')$.
		\item If $v_1$ satisfies condition 3 and $v_2$ satisfies condition 2, define $v'' \gets \prod( r(v_1), v_2)$ and $v' \gets \union( v'', v_2)$.
		\item If both $v_1$ and $v_2$ satisfy condition 3, define $v'' \gets \prod( r(v_1), r(v_2))$, $v_3 \gets \union( v'', r(v_2))$, and $v_4 \gets \union( r(v_1), v_3)$. Lastly, define $\lambda(v') = \cup$, $\ell(v') = \eps$, and $r(v') = v_4$.
	\end{itemize}
	
	One can verify that these constructions work as expected, namely, $\sem{\cD'}(v) = \sem{\cD}(v_1)\cdot\sem{\cD}(v_2)$. Also, if $v_1$ and $v_2$ are $\eps$-safe, then $v'$ is $\eps$-safe as well. Also, each construction does a fixed number of steps, so they take constant time.
	
	\begin{figure}[t]
		\centering
		\hfill
		\begin{tikzpicture}[->,>=stealth',roundnode/.style={circle,draw,inner sep=1.2pt},squarednode/.style={rectangle,inner sep=2pt}, scale=1]
			\node [squarednode] (c) at (1.12, -0.6) {$(a)$};
			\node [squarednode] (0) at (0.8, 2.75) {$\union$};
			\node [squarednode] (6) at (-0.05, 2.75) {$v'\, \colon$};
			\node [squarednode] (1) at (0, 1) {$v_1$};
			\node [squarednode] (2) at (1.6, 1.75) {$\prod$};
			\node [squarednode] (3) at (1.6, 1) {$v_2$};
			\node [squarednode] (4) at (0.8, 0) {$\eps$};
			\node [squarednode] (5) at (2.4, 0) {$r(v_2)$};
			\draw[dashed] (0) to[out=-135,in=90] (1);
			\draw (0) to[out=-45,in=120] (2);
			\draw (2) to[out=-45,in=90] (5);
			\draw[dashed] (3) to[out=-135,in=60] (4);
			\draw (3) to[out=-45,in=120] (5);
			\draw[dashed] (2) to (1);
		\end{tikzpicture} \hfill
		\begin{tikzpicture}[->,>=stealth',roundnode/.style={circle,draw,inner sep=1.2pt},squarednode/.style={rectangle,inner sep=2pt}, scale=1]
			\node [squarednode] (c) at (1.6, -0.6) {$(b)$};
			\node [squarednode] (0) at (2.5, 2.75) {$\union$};
			\node [squarednode] (6) at (1.65, 2.75) {$v'\, \colon$};
			\node [squarednode] (1) at (3, 1) {$v_2$};
			\node [squarednode] (2) at (1.90, 1.75) {$\ \prod$};
			\node [squarednode] (3) at (0.85, 1) {$v_1$};
			\node [squarednode] (4) at (0.2, 0) {$\eps$};
			\node [squarednode] (5) at (1.5, 0) {$r(v_1)$};
			\draw (0) to[out=-60,in=90] (1);
			\draw[dashed] (0) to[out=-135,in=70] (2);
			\draw[dashed] (2) to[out=-120,in=90] (5);
			\draw[dashed] (3) to[out=-135,in=60] (4);
			\draw (3) to[out=-45,in=120] (5);
			\draw (2) to (1);
		\end{tikzpicture} \hfill
		\begin{tikzpicture}[->,>=stealth',roundnode/.style={circle,draw,inner sep=1.1pt},squarednode/.style={rectangle,inner sep=2pt},scale=1.1]
			\node [squarednode] (c) at (1.6, -0.5) {$(c)$};
			\node [squarednode] (0) at (1.5, 2.75) {$\cup$};
			\node [squarednode] (11) at (0.88, 2.8) {$v'\, \colon$};
			\node [squarednode] (1) at (0.75, 2.25) {$\eps$};
			\node [squarednode] (2) at (2.25, 2.25) {$\union$};
			\node [squarednode] (3) at (3, 1.75) {$\union$};
			\node [squarednode] (4) at (2.1, 1) {$\prod$};
			\node [squarednode] (5) at (3.2, 1) {$v_2$};
			\node [squarednode] (6) at (2.5, 0) {$\eps$};
			\node [squarednode] (7) at (4, 0) {$r(v_2)$};
			\node [squarednode] (8) at (0.5, 1) {$v_1$};
			\node [squarednode] (9) at (0, 0) {$\eps$};
			\node [squarednode] (10) at (1, 0) {$r(v_1)$};
			\draw[dashed] (0) to (1);
			\draw (0) to (2);
			\draw[dashed] (2) to[out=-135,in=70] (10);
			\draw[dashed] (4) to (10);
			\draw (4) to[out=-45,in=145] (7);
			\draw[dashed] (5) to[out=-135,in=60] (6);
			\draw (5) to[out=-45,in=120] (7);
			\draw (3) to[out=-45,in=90] (7);
			\draw[dashed] (3) to (4);
			\draw (2) to (3);
			\draw (8) to[out=-50,in=100] (10);
			\draw[dashed] (8) to[out=-125,in=80] (9);
		\end{tikzpicture} \ \ \hfill
		\caption{Gadgets for $\prod$ as defined for a \dsabbr with the $\eps$-node.}
		\label{fig-prod-multi-gadget}
	\end{figure}
	
	%We now address the $\union$ case. To aid the intuition behind these constructions, notice that the \dsabbr structure with the $\eps$-node and the empty-node define sets in $2^{\infAlph^*}$, and can be thought of as the semiring $(2^{\infAlph^*}\!\!, \emptyset, \{\eps\}, \times, \cup)$. In particular 
	
	Similarly, we address the operation $\union(v_3, v_4) \to v'$ by considering each case separately.
	%Since this is a commutative operation, in the sense that the result of $\union( v_3, v_4)$ and $\union( v_4, v_3)$ should define the same set, we only describe the cases where the conditions satisfied by $v_3$ and $v_4$ are $(1,1)$, $(1, 2)$, $(1, 3)$, $(2, 2)$, $(2, 3)$ and $(3, 3)$.
	\begin{itemize}
		\item Assume $v_3$ is the $\eps$-node (condition 1). (1) If $v_4$ also is the $\eps$-node, then we simply return $v'\gets\eps$. (2) If $v_3$ satisfies condition 2, let $v'$ be a union node such that $\ell(v') = \eps$ and $r(v') = v_4$. It can be seen that $v'$ satisfies condition 3 and that its $\eps$-safe. (3) If $v_4$ satisfies condition 3, we simply return $v'\gets v_4$.
		\item Assume $v_3$ satisfies condition 2. (1) If $v_4$ is the $\eps$-node, we return $v'\gets \union( v_4, v_3)$ using the construction for the case (2) in the previous item. (2) If $v_4$ satisfies condition 2, then we return $v'\gets \union( v_3, v_4)$ as it was defined for \dsabbrs without $\eps$. (3) If $v_4$ satisfies condition 3, let $v'' \gets \union( v_3, r(v_4))$, and let $v'$ be a union node such that $\ell(v') = \eps$ and $r(v) = v''$. Again, it can be seen that $v'$ is $\eps$-safe.
		\item Assume $v_3$ satisfies condition 3. (1) If $v_4$ is the $\eps$-node, we simply return $v'\gets\eps$. (2) If $v_4$ satisfies condition 2, we follow the construction given in case (3) of the previous item. (3) If $v_4$ satisfies condition 3, let $v''\gets\union( r(v_3), r(v_4))$ and let $v'$ be a union node such that $\ell(v') = \eps$ and $r(v) = v''$. It can be seen that $v'$ is $\eps$-safe.
	\end{itemize}
	
	Clearly, in each of these cases above we have that $\sem{\cD}(v') = \sem{\cD}(v_3)\cup \sem{\cD}(v_4)$, and if $v_3$ and $v_4$ are $\eps$-safe, then $v'$ is $\eps$-safe as well. In addition, they all take constant time and in each case the new version of $\cD$ satisfies the $\eps$-condition.
	
	The operation $\shiftop( v, k)$ is defined as follows. If $v$ is the $\eps$-node, we return $v'\gets\eps$. If $v$ satisfies condition 2, we return $v'\gets\shiftop( v, k)$ as it was defined for \dsabbrs without $\eps$. If $v$ satisfies condition 3, let $v''\gets\shiftop(r(v), k)$ and let $v'$ be a union node such that $\ell(v') =\eps$ and $r(v) = v''$. It can be seen that $v'$ is $\eps$-safe.
	
	By the previous constructions, we can conclude that the operations $\add$, $\prod$, $\union$ and $\shiftop$, when done over $\eps$-safe nodes, can be done in constant time, return an $\eps$-safe node, maintain the $\eps$-condition in the \dsabbr, and satisfy the specifications of each operation. Furthermore, by virtue of Corollary~\ref{prop:lindelayeps}, the set $\sem{D}(v)$ can be enumerated with output-linear~delay for each node $v$ in $\cD$.

%We summarize the case of $\epsilon$-nodes in the following theorem which is an extension of Theorem~\ref{theo:data-structure}.

\begin{thm}\label{theo:data-structure-eps}
	The operations $\add$, $\prod$, $\union$ and $\shiftop$ over \dsabbr{} extended with empty- and $\epsilon$-nodes take constant time. Furthermore, if we start from an empty \dsabbr{}~$\cD$ and apply $\add$, $\prod$, $\union$, and $\shiftop$ over $\epsilon$-safe nodes, the resulting node $v'$ is always an $\epsilon$-safe node, and the set $\sem{\cD}(v)$ can be enumerated with output-linear delay without preprocessing for every node $v$.
\end{thm} 

For the rest of the paper, we assume that a \dsabbr{} is a tuple $\cD = (\infAlph, V, \lch, \rch, \lambda, \bot, \epsilon)$ where we define $\infAlph, V, \lch, \rch,\lambda$ as before, and $\bot, \epsilon \in V$ are the empty- and $\epsilon$-node, respectively. Further, we assume that $\lch$, $\rch$, and $\lambda$ are extended accordingly, namely,  $\lch(v)$ and $\rch(v)$ are not defined whenever $v \in \{\bot, \epsilon\}$, and $\lambda:V\to\infAlph\cup\int \cup \{\cup, \odot,\bot, \eps\}$ such that $\lambda(v) = \bot$ ($\lambda(v) = \epsilon$) iff $v = \bot$ ($v = \eps$, respectively). 
%Finally, we can extend Theorem~\ref{theo:data-structure} for the \dsabbr{} extension as follows. 






==> sections/edits.tex <==
%!TEX root = ../main/main.tex
% !TeX spellcheck = en_US

\newcommand{\rS}{\hat{S}}

In this section, we show that the results obtained by Schmid and Schweikardt~\cite{SchmidS22} regarding enumeration over document databases and complex document editing still hold, maintaining the same time bounds in doing these edits, but allowing output-linear delay. We also include a refinement of the result for whenever the edits needed are limited to the concatenation of two documents. 

\cristian{Arreglar la intro anterior.}

\paragraph{Complex Document Editing}
A document database over $\Sigma$ is a finite collection of documents over $\Sigma$ where each document has a name. Formally, a \emph{document database} is a function $D: \{d_1, \ldots, d_m\} \rightarrow \Sigma^*$ where $\{d_1, \ldots, d_m\}$ is a finite set of \emph{documents names} and $D(d_i)$ is the document assigned to the name $d_i$. We also say that $\{d_1, \ldots, d_m\}$ is the \emph{schema} of the document database $D$. 

Given a document database $D$ our goal is to create new documents by a sequence of text-editing operations.
Here, we introduce the notion of a \emph{Complex Document Editing expression} (CDE-expression for short) over document names $\{d_1, \ldots, d_m\}$, which is defined by the following \emph{syntax}:
\[
\renewcommand{\arraystretch}{1.2}
\begin{array}{rcl}
	\varphi & := &  d_\ell, \ell\in[1, m] \\
	 & \mid &  \concat(\varphi, \varphi) \\
	 & \mid &  \extract(\varphi, i, j) \\
	 & \mid &  \delete(\varphi, i, j) \\
	 & \mid &  \insertop(\varphi, \varphi, k) \\
	 & \mid & \copyop(\varphi, i, j, k)
\end{array}
\]
where the values $i,j$ are valid {\it positions}, and $k$ is a valid {\it gap}. % -- concepts that we will explain shortly. 
We define $|\varphi|$ as the number of basic operations in $\varphi$.

The \emph{semantics} of an CDE-expression $\varphi$ defines a function $\sem{\varphi}$ from document databases over $\{d_1, \ldots, d_m\}$ to documents, and works recursively as follows:
\[
\renewcommand{\arraystretch}{1.4}
\begin{array}{rcl}
	\sem{d_\ell}(D) & = & D(d_\ell) \\
	\sem{\concat(\varphi_1, \varphi_2)}(D) & = & \sem{\varphi_1}(D) \cdot \sem{\varphi_2}(D)  \\
	\sem{\extract(\varphi, i, j)}(D) & = & \sem{\varphi}(D)\spanc{i}{j+1} \\
	\sem{\delete(\varphi, i, j)}(D) & = & \sem{\varphi}(D)\spanc{1}{i} \cdot \sem{\varphi}(D)\spanc{j+1}{|\sem{\varphi}(D)|+1} \\
	\sem{\insertop(\varphi_1, \varphi_2, k)}(D) &=& \sem{\varphi_1}(D)\spanc{1}{k}\cdot \sem{\varphi_2}(D) \cdot \sem{\varphi_1}(D)\spanc{k}{|d|+1} \\
	\sem{\copyop(\varphi, i, j, k)}(D) &=& \sem{\varphi}(D)\spanc{1}{k}\cdot \sem{\varphi}(D)\spanc{i}{j+1} \cdot \sem{\varphi}(D)\spanc{k}{|\sem{\varphi}(D)|+1} 
\end{array}
\]
where $\varphi$, $\varphi_1$, and $\varphi_2$ are CDE-expressions, $i,j$ are valid positions, and $k$ is a valid gap. We assume that if $i$, $j$, or $k$ are not valid, then $\sem{\varphi}(D)$ is undefined. Since verifying that positions are valid for $\varphi$ takes linear time in $|D|$ and $|\varphi|$, for the sake of simplification we assume that positions and gaps are always valid. 

The complex document editing operations were formally introduced in~\cite{SchmidS22}, and here we present an equivalent formalization of such framework that better fits our purposes. As the name of each operation suggested, $\concat$ defines the concatenation of two documents, $\extract$ outputs the span $\spanc{i}{j+1}$ of a document, $\delete$ removes the substring in the span $\spanc{i}{j+1}$,  $\insertop$ adds a document inside the other at position $k$, and $\copyop$ inserts the substring at the span $\spanc{i}{j}$ at the position $k$.
See~\cite{SchmidS22} for several example and applications for CDE-expressions.

\paragraph{Multiroot SLPs}
A \emph{multiroot SLP} is a tuple $\rS = (N, \Sigma, R, \rS_0)$ where $N$ is a set of non-terminals, $\Sigma$ is the set of terminals, $R$ is a set of rules, and $\rS_0: \{d_1, \ldots, d_m\} \rightarrow N$ maps document names to non-terminals. Further, we suppose that $\rS(d_i) = (N, \Sigma, R, \rS_0(d_i))$ forms an SLP with start symbol $\rS_0(d_i)$. In other words, $\rS$ is like an SLP but with multiple roots $\rS_0(d_1), \ldots, \rS_0(d_m)$. 

A multiroot SLP $\rS$ naturally defines a document database that maps each document name $d_i$ to $\doc(\rS(d_i))$. By some abuse of notation, we write $\doc(\rS)$ to denote the document database $\doc(\rS): \{d_1, \ldots, d_m\} \rightarrow \Sigma^*$ such that $[\doc(\rS)](d_i) = \doc(\rS(d_i))$.   Therefore, multiroot SLPs work as our formalism to specify compressed document databases where we can apply CDE-expressions. We naturally extend the semantics of a CDE-expression $\varphi$ from database documents to multiroot SLPs as $\sem{\varphi}(\rS) = \sem{\varphi}(\doc(\rS))$ where $\varphi$ is over $\{d_1, \ldots, d_m\}$.

\paragraph{The query evaluation problem} 
We are ready for defining the query evaluation problem of complex editing expressions over compressed document databases. Let $\mathcal{C}$ be any class of \crt and $\mathcal{E}$ any class of CDE-expressions (e.g., expressions that only uses $\concat$). 

\begin{center}
	\framebox{
		\begin{tabular}{rl}
			\textbf{Problem:} \!\!\!\!\!\!& $\enumedit[\mathcal{C}, \mathcal{E}]$  \\ \hline \vspace{-3mm} \\
			\textbf{Preprocessing:}  \!\!\!\!\!\! & 
			$\left\{ \text{\begin{tabular}{rl}
					\textbf{input:} & \!\!\! An \crt $\cA \in \mathcal{C}$ and a multiroot-SLP $\rS$ \\
					%                                \textbf{output:}
					\textbf{result:}
					& \!\!\! A data structure $\DS_{\cA,\rS}$
			\end{tabular}} \right.
			$            \\ \hline \vspace{-3mm} \\
			\textbf{Editing:}  \!\!\!\!\!\! & 
			$\left\{ \text{\begin{tabular}{rl}
					\textbf{input:} & \!\!\! The data structure $\DS_{\cA,\rS}$ and an CDE-expression $\varphi \in \mathcal{E}$ \\
					%                                \textbf{output:}
					\textbf{result:}
					& \!\!\! A data structure $\DS_{\cA,\rS, \varphi}$
			\end{tabular}} \right.
			$            \\ \hline \vspace{-3mm} \\
			\textbf{Enumeration:} \!\!\!\!\!\! &
			$\left\{
			\!\!\text{
				\begin{tabular}{rl}
					\textbf{input:} & \!\!\!
					The data structure $\DS_{\cA,\rS, \varphi}$ \\
					\textbf{output:} & \!\!\! Enumerate $\sem{\cA}(\sem{\varphi}(\doc(\rS)))$
				\end{tabular} 
			}\right.$\!\!\!\!
		\end{tabular}
	}
\end{center}

The evaluation problem $\enumedit$ is an extension of the problem $\enumraa$ studied in the previous sections, in the sense that it also has preprocessing and enumeration phases that work as before. The main difference is a middle phase, called \emph{editing}, where we can receive any CDE-expression $\varphi$ for evaluating the \crt $\cA$ over the new document $\sem{\varphi}(\doc(\cA))$. Specifically, the editing phase receives the data structure $\DS_{\cA, \rS}$ of the preprocessing phase plus a CDE-expression $\varphi$. Then it produces a new data structure $\DS_{\cA, \rS, \varphi}$ that will be used later in the enumeration phase of $\sem{\cA}(\sem{\varphi}(\doc(\rS)))$ (i.e., it encode the outputs). 
In other words, the task is to evaluate $\cA$ efficiently over any edited document from the document database without re-processing the data. 
We say that an algorithm for $\enumedit$ has \emph{$g$-preprocessing time} if there exists a constant $c$ such that, for every input $(\cA, \rS, \varphi)$, the time for the editing phase of $\varphi$ is bounded by $c \cdot g(\cA, \rS, \varphi)$. Note that, for doing a fine-grained analysis of the editing running time, we consider all inputs $(\cA, \rS, \varphi)$ given that the data structure $\DS_{\cA,\rS}$ depends on $\cA$ and $\rS$.

It is important to note that this setting is equivalent to the setting presented in~\cite{SchmidS22}. The main difference is in the presentation, where we are more explicit in the semantics of CDE-expressions and in formalizing the preprocessing, editing, and enumeration phases. In~\cite{SchmidS22}, the authors also considered that the input for the preprocessing phase can have several queries $\cA_1, \ldots, \cA_k$ that the user wants to evaluate simultaneously. For the sake of presentation, we adopt the setting with a single query (i.e., an \crt) since one can naturally extend our setting to $k$-queries assuming an additional $k$ factor in the running time of the preprocessing and editing phase. Finally, our setting has the advantage that we consider \crt as input, which is more general than in~\cite{SchmidS22}, where they consider extended variable-set automata.

We are almost ready for presenting the main result of this section. Towards this goal, we need a couple of new definition for multiroot SLPs. We say that a multiroot SLP $\rS = (N, \Sigma, R, \rS_0)$ is in {\it Chomsky normal form} (or just normal form) if every rule in $R$ has the form $X\to a$ or $X\to YZ$, where $a\in \Sigma$ and $X, Y, Z\in N$. Also, we say that $\rS$ is {\it strongly balanced} if it is in Chomsky normal form and, for each rule $X\to YZ$, the value $\ord(Y) - \ord(Z)$ is either -1, 0 or 1, where $\ord(X)$ is the maximum distance from $X$ to any terminal in the derivation tree.  We define the {\it maximum intermediate document size} $|\max_{\varphi}(D)|$ induced by a CDE-expression $\varphi$ on a document database $D$ as the maximum size of $\sem{\psi}(D)$ for any sub-expression $\psi$ of $\varphi$ (i.e., any substring $\psi$ of $\varphi$ that matches the CDE syntax).

\begin{thm}\label{theo:edit-main-theorem}
	Let $\mathcal{C}$ be the class of all unambiguous \rts and $\mathcal{E}$ the class of all CDE-expressions. Assuming that the input multiroot SLP $\rS$ is strongly balanced, one can solve $\enumedit[\mathcal{C}, \mathcal{E}]$ with $|\cA|^3 \times |S|$-preprocessing time, $|\varphi| \times |\cA|^3  \times \log|\max_{\varphi}(\doc(\rS))|$-editing time, and output-linear delay.  
\end{thm}

The version of this result shown in~\cite{SchmidS22} had extended VA instead of \crt, and logarithmic delay instead of output-linear delay. The proof goes by combining the techniques of~\cite{SchmidS22} for editing SLPs and the machinery developed in the previous sections.
\begin{proof}
	Let $\rS = (N, \Sigma, R, \rS_0)$ be a strongly balanced multiroot SLP and $\cA = (Q, \Sigma, \oalph, \Delta, \qinit, F)$ be an unambiguous \crt. In a nutshell, the algorithm strategy is as follows: During the preprocessing phase, we construct the succinct \dsabbr $\cD$ and the set of matrices $\{M_X\}_{X \in N}$ associated with $\rS$ and $\cA$ (i.e., by running Algorithm~\ref{alg:evaluation}). Then, during the editing phase, we extend $\rS$ to a multiroot SLP $\rS'$ by adding new non-terminals $N'$ (and rules over $N'$) that represent partial documents of evaluating $\varphi$ with special non-terminal $S_0'$ representing the document $\sem{\varphi}(\rS)$. For each new non-terminal $X' \in N'$, we construct its matrix $M_{X'}$ extending $\cD$ to $\cD'$. Finally, we enumerate the results with output-linear delay using $\cD'$ and the matrix $M_{S_0'}$ similar to in Algorithm~\ref{alg:evaluation}. 
	
	We start by showing how to do the extension of $\rS$ to $\rS'$ by using $\varphi$.
	In the following, we assume that for each nonterminal $X$ of $\rS$ for which its rule has the form $X\to YZ$, the values $|\doc(X)|$, $\ord(X)$, and nonterminals $Y$ and $Z$ are accessible in constant time. 
	All these values can be precomputed with a linear-time pass over $\rS$ during the preprocessing. We call $\rS$ along with constant-time access to these values {\it the basic data structure for} $\rS$.
	Furthermore, a multiroot SLP $\rS' = (N \cup N', \Sigma, R', \rS'_0)$ is called an \emph{extension} of $\rS$ if $R'(A) = R(A)$ for every $A\in N$. In this context, we call $N'$ the {\it set of new non-terminals}.
	
	The following result from~\cite{SchmidS22} will be instrumental in the proof. 
	\begin{thmC}[(Theorem 4.3 in \cite{SchmidS22})]\label{theo:cedits}
		Let $\rS$ be a strongly balanced multiroot SLP with document names $\{d_1, \ldots, d_m\}$. When given the basic data structure for $\rS$ and a CDE-expression $\varphi$ over $\{d_1, \ldots, d_m\}$, we can construct a strongly balanced extension $\rS'$ of $\rS$, along with its basic data structure, and a non-terminal $S_0'$ of $\rS'$ such that $\doc(S_0') = \sem{\varphi}(\rS)$.
		This construction takes time $\cO\big(|\varphi|\cdot \log|\max_{\varphi}(\doc(\rS))|\big)$.  In particular, the number of new non-terminals $|N'|$ is in $\cO\big(|\varphi|\cdot \log|\max_{\varphi}(\doc(\rS))|\big)$.
	\end{thmC}
	
	Let $\cD$ be the succinct \dsabbr and $\{M_X\}_{X \in N}$ the set of matrices associated to $\rS$ and $\cA$ after the preprocessing phase. Further, let $\tilde{R} = R' \setminus R$ be the set of new rules in $\rS'$ after applying Theorem~\ref{theo:cedits}. Consider the DAG that is induced by this set $\tilde{R}$. We can go over these new rules $X'\to Y'Z'$ in a bottom-up fashion, starting from the ones where $Y',Z'\in N$, and define the nodes $M_{X'}[p,q] = (M_{Y'}\otimes \shiftop(M_{Z'},|\doc(Y')|))[p,q]$ for each $p,q\in Q$. Then, we build the nodes $v_{X'}$ for each new non-terminal $X'$ as defined. The new nodes are created by application of the \dsabbr operations $\add$, $\union$, $\prod$ and $\shiftop$ which create the succinct \dsabbr $\cD'$ that defines the query data structure for $\rS'$ and $\cA$. The procedure takes $\cO(|Q|^3\cdot|N'|)$ time. By Theorem~\ref{theo:cedits}, this means that the editing time is in $\cO\big(|Q|^3 \cdot |\varphi|\cdot \log|\max_{\varphi}(\doc(\rS))|\big)$.
	Finally, we can use the matrix $M_{S_0'}$ and the nodes at entries $(p, q) \in I \times F$ for retrieving the outputs with output-linear delay during the enumeration phase.
\end{proof}

It is important to notice that we assume that $\rS$ is strongly balanced and use Theorem 4.3 in \cite{SchmidS22} to bound the number of new nonterminals that are necessary to implement the operations $\extract$, $\delete$, $\insertop$, and $\copyop$ of CDE-expressions. In \cite{SchmidS22}, the strongly balanced condition was also needed for enforcing the log-delay during enumeration, which is not the case here. In particular, we can get the following result if we assume that our CDE-expressions only uses the $\extract$ operation.   

\begin{corollary}\label{cor:concat}
	Let $\mathcal{C}$ be the class of all unambiguous \rts and $\mathcal{E}$ the class of all CDE-expressions that only uses document names and $\concat$ operation. One can solve $\enumedit[\mathcal{C}, \mathcal{E}]$ with $|\cA|^3 \times |S|$-preprocessing time, $|\varphi| \times |\cA|^3 $-editing time, and output-linear delay.  
\end{corollary}

\begin{proof}
	The proof follows the same lines than in Theorem~\ref{theo:edit-main-theorem}. The difference is that we do not need Theorem~\ref{theo:cedits} since the concatenation operation can be done directly adding a new non-terminal for each $\concat$ operation. In particular, the number of new non-terminals $|N'|$ is~in~$\cO(|\varphi|)$. 
\end{proof}


\cristian{PREVIOUS VERSION}

In this section, we show that the results obtained by Schmid and Schweikardt~\cite{SchmidS22} regarding enumeration over document databases and complex document editing still hold, maintaining the same time bounds in doing these edits, but allowing output-linear delay. We also include a refinement of the result for whenever the edits needed are limited to the concatenation of two documents. To be precise, we will give an overview of the following theorem.

\begin{thm}\label{theo:edits}
	Let $D = \{d_1,\ldots,d_m\}$ be a document database that is represented by an SLP~$S$ in normal form. Let $\cA_1,\ldots,\cA_k$ be unambiguous sequential variable-set automata. When given the query data structures for $S$ and $\cA_1,\ldots, \cA_k$, and a CDE-expression $\varphi$ over $D$, we can construct an extension $S'$ of $S$ and new query data structures for $S'$ and $\cA_1,\ldots,\cA_k$, and a new non-terminal $\tilde{A}$ of $S'$, such that $\doc(\tilde{A}) = \textsf{eval}(\varphi)$. 
	\begin{itemize}
		\item If $\varphi$ contains operations other than $\concat$, we require $S$ to be strongly balanced. Then, $S'$ is also strongly balanced, and this construction can be done $\cO(k\cdot|\varphi|\cdot\log|d^*|)$ time in data-complexity where $|d^*| = |\max_{\varphi}(D)|$.
		\item If $\varphi$ only contains $\concat$, then this can be done in $\cO(k\cdot|\varphi|)$ time in data-complexity.
	\end{itemize}
	Afterwards, upon input of any $d\in\docs(S')$ (represented by a non-terminal of $S'$) and any $i\in[1, m]$, the set $\sem{\cA_i}(d)$ can be enumerated with constant-delay.
\end{thm}

The version of this result shown in~\cite{SchmidS22} had extended VA instead of VA, and logarithmic delay instead of constant-delay.
We dedicate the rest of this section to define the concepts we have not yet introduced in Theorem~\ref{theo:edits}, and show how the techniques presented in~\cite{SchmidS22} allow us to obtain this result. 
%From what we have seen so far, this is not obviously an improvement of Theorem 6.4 from~\cite{SchmidS22} because we have not yet presented a rigorous link between annotated automata and regular spanners. This is done in Section~\ref{sec:spanners}, where the result is also extended to support several spanners to match Schmid and Schweikardt's result.

\paragraph{Normal form, balanced and rootless SLPs}
 We define a {\it rootless SLP} as a triple $S = (N, \Sigma, R)$, where $N$ is a set of non-terminals, $\Sigma$ is the set of terminals, and $R$ is a set of rules. Rootless SLPs are defined as SLPs with the difference that there is no starting symbol, and thus $\doc(S)$ is not defined. Instead, we define $\doc(A)$ for each $A\in N$ as $\doc(A) = R^*(A)$. We say that $S$ is in {\it Chomsky normal form} (or just normal form) if every rule in $R$ has the form $A\to a$ or $A\to BC$, where $a\in \Sigma$ and $A, B, C\in N$. Also, we say that $S$ is {\it strongly balanced} if for each rule $A\to BC$, the value $\ord(B) - \ord(C)$ is either -1, 0 or 1, where $\ord(X)$ is the maximum distance from $X$ to any terminal in the derivation tree. 

\paragraph{Document Databases} 
A {\it document database} over $\Sigma$ is a finite collection $D = \{d_1, \ldots, d_m\}$ of documents over $\Sigma$. Document databases are represented by a rootless SLP as follows. For an SLP $S = (N, \Sigma, R)$, let $\docs(S) = \{\doc(A)\mid A\in N\}$ be the set of documents represented by $S$. The rootless SLP $S$ is a representation for a document database $D$ if $D\subseteq \docs(S)$.

For a document database $D$, it is assumed that a rootless SLP $S$ that represents $D$ is in normal form and, for the effects of the first bullet point of Theorem~\ref{theo:edits}, strongly balanced. It is also assumed that for each nonterminal $A$ for which its rule has the form $A\to BC$, the values $|\doc(A)|$, $\ord(A)$ and nonterminals $B$ and $C$ are accessible in constant time. 
All these values can be  precomputed with a linear-time pass over $S$. We call $S$ along with constant-time access to these values {\it the basic data structure for} $S$.

\paragraph{Complex Document Editing}
As in~\cite{SchmidS22}, given a document database $D = \{d_1, \ldots, d_m\}$ our goal is to create new documents by a sequence of text-editing operations.
Here we introduce the notion of a CDE-expression over $D$, which is defined by the following syntax:
\[
	\varphi := \ d_\ell, \ell\in[1, m]\ | \ \concat(\varphi, \varphi)\ | \ \extract(\varphi, i, j) \ | \
	\delete(\varphi, i, j) \ | \ \insertop(\varphi, \varphi, k) \ | \ \copyop(\varphi, i, j, k)
\]
where the values $i,j$ are valid {\it positions}, and $k$ is a valid {\it gap}. % -- concepts that we will explain shortly. 
The semantics of these operations, called {\it basic operations}, works as follows:
\[
\begin{array}{rclrclrclrcl}
	\concat(d, d') &=& d\cdot d' \ \ \ &&\insertop(d, d', k) &=& d\spanc{1}{k}\cdot d'\cdot d\spanc{k}{|d|+1}&\\
	\extract(d, i, j) &=& d\spanc{i}{j+1} \ \ \ &&\delete(d, i, j) &=& d\spanc{1}{i}\cdot d\spanc{j+1}{|d|+1}&\\
	\copyop(d, i, j, k) &=& \insertop(d, d\spanc{i}{j+1}, k) 	
	%	&=&d\spanc{i}{k}\cdot d\spanc{i}{j+1}&\cdot& d\spanc{k}{|d|+1} \  \ \ \ \ \ \ \ \ \ \ \ \ \ &
\end{array}
\]
We write $\eval(\varphi)$ for the document obtained by evaluating $\varphi$ on $D$ according to these semantics. For an operation $\extract(\varphi, i, j)$, $\delete(\varphi, i, j)$, $\insertop(\varphi, \psi, k)$, or $\copyop(\varphi, i, j, k)$, $i,j$ are valid positions if $i, j\in [1, |\eval(\varphi)|]$, and $k$ is a valid gap if $k\in [1, |\eval(\varphi)| + 1]$.
We define $|\varphi|$ as the number of basic operations in $\varphi$.
For adding these new documents in the database we will use the notion of extending a rootless SLP. A rootless SLP $S' = (N', \Sigma, R')$ is called an extension of $S$ if $S'$ is in normal form, $N\subseteq N'$, and $R'(A) = R(A)$ for every $A\in N$. In this context, we call $N'\setminus N$ the {\it set of new non-terminals}.
We define the {\it maximum intermediate document size} $|\max_{\varphi}(D)|$ induced by a CDE-expression $\varphi$ on a document database $D$ as the maximum size of $\eval(\psi)$ for any sub-expression $\psi$ of $\varphi$ (i.e., any substring $\psi$ of $\varphi$ that matches the CDE syntax).

%At this point we have covered all definitions needed in the statement of Theorem~\ref{theo:edits}. We need one more tool from~\cite{SchmidS22} which will be what we need to prove this theorem.

Having defined most of the concepts mentioned in Theorem~\ref{theo:edits}, we can re-state the following Theorem from~\cite{SchmidS22}, which will be instrumental in the final proof.

\begin{thmC}[(Theorem 4.3 in \cite{SchmidS22})]\label{theo:cedits}
	Let $D$ be a document database represented by a strongly balanced rootless SLP $S$ in normal form. When given the basic data structure for $S$ and a CDE-expression $\varphi$ over $D$, we can construct a strongly balanced extension $S'$ of $S$, along with its basic data structure, and a non-terminal $\tilde{A}$ of $S'$ such that $\doc(\tilde{A}) = \eval(\varphi)$.
	This construction takes time $\cO\big(|\varphi|\cdot \log(|\max_{\varphi}(D)|)\big)$.  In particular, the number of new non-terminals $|N'\setminus N|$ is in $\cO\big(|\varphi|\cdot \log( |\max_{\varphi}(D)|)\big)$.
\end{thmC}

%To give an idea of the strategy for the proof, we will start from a {\it query data structure} built over some rootless SLP $S$ and an \rtname $\cA$, extend $S$ into another SLP $S'$, and then extend this query data structure so it is defined over $S'$ and $\cA$. The time this takes depends only on the number of new non-terminals in $S'$ and on $\cA$.

For the second bullet point in Theorem~\ref{theo:edits}, we use the following observation, which comes from the fact that applying $\concat$ to an SLP amounts to adding a single production.

\begin{obs}\label{obs:concat}
	Let $D$ be a document database represented by a rootless SLP $S$ in normal form. Given the basic data structure for $S$ and a CDE-expression $\varphi$ over $D$ which only mentions $\concat$, we can construct an extension $S'$ of $S$, along with its basic data structure, and a nonterminal $\tilde{A}$ of $S'$ such that $\doc(\tilde{A}) = \eval(\varphi)$. This construction takes time $\cO(|\varphi|)$. In particular, the number of new non-terminals $|N'\setminus N|$ is~in~$\cO(|\varphi|)$.
\end{obs}

\paragraph{The query data structure}
The structure we will use is the one produced in Theorem~\ref{theo-algo-succ}. This structure is built by an algorithm that receives an SLP $S$, an unambiguous \crt $\cA$, and produces a succinct \dsabbr $\cD$ indexed by the matrices $M_A$, for each non-terminal $A$ in~$S$. These matrices store nodes $v = M_A[p,q]$ such that $\sem{\cD}(v)$ contains all partial annotations from a path of $\cA$ which starts $p$, ends in $q$, and reads the string $\doc(A)$. 
Note that, although the algorithm receives a ``rooted'' SLP, it can be adapted quite easily to rootless SLPs by adding a node $v_A$ for each non-terminal $A$ in $S$, built as $v_A = \union_{q\in F}(M_A[q_0, q])$ (the same construction that was done for $S_0$ in the algorithm).

We define {\it the query data structure for $S$ and $\cA$} as the mentioned succinct \dsabbr along with constant-time access to every index $M_A[p,q]$ for states $p$ and $q$ and non-terminal~$A$. Note that for each $A$ it holds that $\sem{\cD}(v_A) = \sem{\cA}(\doc(A))$. In particular, if $S$ represents a document database $D$, then for each $d\in D$ there is a $v$ in $\cD$ for which $\sem{\cD}(v) = \sem{\cA}(d)$. Recall that for every node $v\in \cD$, the set $\sem{\cD}(v)$ can be enumerated with output-linear delay.

\begin{lem}\label{lem:ecsext}
	Let $S$ be an SLP in normal form and an extension $S'$ of $S$ with new non-terminals $\tilde{N} = N' \setminus N$. Also, let $\cA$ be an unambiguous \crt and assume we are given the query data structure for $S$ and $\cA$, and the basic data structure for $S'$. We can construct the query data structure for $S'$ and $\cA$ in $\cO(|\cA|^3\cdot|\tilde{N}|)$ time.
\end{lem}
\begin{proof}
	Let $\cD$ be the succinct \dsabbr associated to the query data structure for $S$ and $\cA$ and let $\tilde{R} = R' \setminus R$ be the set of new rules in $S'$. Consider the DAG that is induced by this set. We can go over these new rules $\tilde{A}\to BC$ in a bottom-up fashion, starting from the ones where $B,C\in N$, and define the nodes $M_{\tilde{A}}[p,q] = (M_{B}\otimes \shiftop(M_C,|\doc(B)|))[p,q]$ for each $p,q\in Q$. Then, we build the nodes $v_{\tilde{A}}$ for each new non-terminal $\tilde{A}$ as defined. The new nodes are created by application of the \dsabbr operations $\add$, $\union$, $\prod$ and $\shiftop$ which create the succinct \dsabbr $\cD'$ that defines the query data structure for $S'$ and $\cA$. The procedure takes $\cO(|Q|^3\cdot|\tilde{N}|)$ time.
\end{proof}

We finally have all the machinery to prove Theorem~\ref{theo:edits}, extending the results in~\cite{SchmidS22} for sequential VA and with output-linear delay.

\paragraph{Proof of Theorem~\ref{theo:edits}} Let us first reduce the variable-set automata $\cA_1, \ldots \cA_k$ to \crt{}s $\cA_1',\ldots,\cA_k'$ using the construction of Proposition~\ref{prop:va-reduc}. Note, however, that this reduction requires the input document to be modified as well. This can be solved by adding a non-terminal $A_{\texttt{\#}}$ for each $A\in N$, and a rule $A_{\texttt{\#}}\to AH$, where $H$ is a new non-terminal with the rule $H\to\texttt{\#}$. Then, in the query data structure for $S$ and $\cA'$, the nodes $v_A$ are defined over the matrices $M_{A_{\texttt{\#}}}$ instead. That way, when the user chooses a document $d\in \docs(S)$ and a variable set automata $\cA_i$, she can be given the set $\sem{\cA'_i}(d\texttt{\#})$ as output. Note that this has no influence in the time bounds given for the edit so far, except for a factor that is linear~in~$|\tilde{N}|$.

We can see now that the result follows from Theorem~\ref{theo:cedits}, Observation~\ref{obs:concat}, and Lemma~\ref{lem:ecsext}. The fact that for each $d\in \docs(S')$ the set $\sem{\cA}(d)$ can be enumerated with output-linear delay follows from the definition of the query data structure for $S'$ and $\cA$. \qed
%-- one must simply use the node $v_A$ for the non-terminal $A$ that satisfies $\str(A) = d$, and note that, by virtue of Theorem~\ref{theo:data-structure-eps}, the set $\sem{\cD}(v_A) = \sem{\cA}(d)$ can be enumerated as mentioned.

==> sections/enum.tex <==
%!TEX root = main.tex

An enumeration problem is defined as a relation $R\subseteq \Omega_{in} \times \Omega_{out}$ for some set of inputs $\Omega_{in}$ and some set of outputs $\Omega_{out}$.
For each pair $(x, y)\in R$ we view $x$ as the input of the problem and $y$ as a possible output for $x$.
We define the set $R(x) = \{y\mid(x, y)\in R\}$ as the set of outputs of $x$.

An enumeration algorithm $\mathfrak{A}$ for $R$ is one that operates in two phases: First, $\mathfrak{A}$ receives an input $x$, and builds a certain object $D_x$ which can be used to retrieve the set $R(x)$ -- we call this phase the preprocessing phase. Then, $\mathfrak{A}$ performs a subroutine $\yield$ over $D_x$ to retrieve $R(x)$. There is also a constant value $c$ which is fixed for the algorithm. The subroutine $\yield$ has the following specifications: (1) it can be done immediately over the object $D_x$ for any input $x$, (2) It can be done exactly $|R(x)|+1$ times over $D_x$, (3) the first $|R(x)|$ applications of $\yield$ over $D_x$ produces a different element $y\in R(x)$ and (4) the last application of $\yield$ produces a flag ${\tt end}$.

In an enumeration algorithm, we measure the time taken in the preprocessing phase by a function that depends on $x$, which is the time that it takes to produce the object $D_x$. 
We also measure the delay, which gives a bound in the time that passes from the moment any of the calls to $\yield$ is made, until an output from $R(x)$ is fully produced -- we refer to this as the time that this call takes.
Asymptotically, the best delay possible is constant delay, which means that there is a constant value $c$ associated to $\mathfrak{A}$ such that the time that any call to $\yield$ takes is at most $c$. Under a reasonable assumption, constant-delay is limited to only problems in which each element in $R(x)$ has bounded size for any input $x$. We will look at an extension of this notion, called output-linear delay, which is still permissible when outputs have unbounded size. Here, any call to $\yield$ takes at most $c\cdot|y|$ time, where $y\in R(x)$ is the output produced.


%By design, enumeration problems are expected to be solved by an algorithm that works in two phases: first, a preprocessing phase in which it receives the input and produces some object $D$ (e.g. a collection of indices, or some new data structure) which stores the expected outputs somehow, and then an enumeration phase which extracts the outputs through $D$.
%In this paper we will not only look at enumeration algorithms as a solution to a two-part problem, instead we will also be interested in accepting these objects $D$ as part of an input.
%Another consideration we will have is that we will only talk about output-linear delay as our gold standard for enumeration efficiency. 
%This is a refinement of the better-known constant-delay bound, which requires (by a reasonable assumption) that each output has constant size. 
%Output-linear delay is the natural extension of this notion which allows outputs of unbounded size, which requires the delay to be bounded linearly in the size of the current output.
%More generally, we will look at classes of objects which allow output-linear delay enumeration as schemes which efficiently represent sets of outputs.
%We can subsequently define enumeration algorithms as those which receive an input, and produce one such scheme.

%Dealing with these objects has to be done with a certain degree of care, since it is easy to miss where the coefficients should come from, and how general they should be.



==> sections/ra.tex <==
%!TEX root = main.tex

In this section, we present the definition of \rtname, which is an extension of regular automata to produce outputs. We use \rtnames as our computational model to represent queries with output. 
	
	A \emph{\rtname} (\rt for short) is a tuple $\cA = (Q, \Sigma, \oalph, \Delta, \qinit, F)$ where $Q$ is a state set, $\Sigma$ is an input alphabet, $\oalph$ is an output alphabet, $\qinit \subseteq Q$ and $F \subseteq Q$ and $\Delta \subseteq Q \times (\Sigma \times \oalph) \times Q \,\cup\, Q \times \Sigma \times Q $ is the transition relation, which contains {\em read-write transitions} of the form $(p, (a, \oout), q)\in Q\times(\Sigma\times\oalph)\times Q$, and {\em read transitions} of the form  $(p, a, q)\in Q\times\Sigma\times Q$.
	
	As usual for transducers, a symbol $a \in \Sigma$ is an input symbol that the machine reads and $\oout \in \oalph$ is a symbol that indicates what the machine prints in an output tape.
	A run $\rho$ of $\cA$ over a document $d = a_1a_2\ldots a_n \in\Sigma^*$ is a sequence of the form
	$
	%\rho = (q_1, \sigma_1) \xrightarrow{s_1/\!\ooutscr_1} (q_2, \sigma_2) \xrightarrow{s_2/\!\ooutscr_2} \ldots  \xrightarrow{s_n/\!\ooutscr_n} (q_{n+1}, \sigma_{n+1})
	\rho = q_0 \xrightarrow{b_1} q_1 \xrightarrow{b_2} \ldots \xrightarrow{b_n} q_{n}
	$
	where $q_0 \in I$, and for each $i\in [1,n]$ one of the following holds: (1) $b_i = a_i$ and there is a transition $(q_{i-1}, a_i, q_i)\in \Delta$ or (2) $b_i = (a_i, \oout)$ and there is a transition $(q_{i-1}, a_i, \oout, q_i)\in \Delta$. We say that $\rho$ is accepting if $q_n\in F$.
	
	Finally, we define the {\em annotation} of $\rho$ as:
	$
	\ann(\rho) =  \ann(b_1)\cdot \ldots \cdot \ann(b_n)
	$
	such that $\ann(b_i) = (\oout, i)$ if $b_i = (a, \oout)$, and $\ann(b_i) = \eps$ otherwise, for each $i\in[1, n]$.
	%Note that in $\nu = \oout_1 \cdots \oout_n$, $\oeps$ is a symbol that may be present in the word, whereas $\eps$ indicates an empty word. 
	Given a \rtname $\cA$ and a document $d \in\Sigma^*$, we define the set $\sem{\cA}(d)$ of all outputs of $\cA$ over $d$ as:
	%$$
	%\sem{\cA}(w) \ = \ \{ \out(\rho) \, \mid \, \text{$\rho$ is an accepting run of $\cA$ over $w$}\}.
	%$$
	$
	\sem{\cA}(d) = \{ \ann(\rho) \, \mid \, \text{$\rho$ is an accepting run of $\cA$ over $d$}\}.
	$
	
	
	We say that a \rt $\cA = (Q, \Sigma, \oalph, \Delta, \qinit, F)$ is %\emph{input/output deterministic} (I/O-deterministic for short) 
	{\it deterministic} if $|\qinit| = 1$ and $\Delta$ is a partial function of the form $\Delta: (Q \times \Sigma \, \cup\, Q\times (\Sigma\times\oalph)) \to Q$.
	%for each triple $(p, a, \oout) \in Q \times \opS \times \oalph$,  there is at most one tuple $(q, \mathtt{x}) \in Q \times \Gamma$ such that $(p, a, \oout, q, \mathtt{x})\in\Delta$, 
	%for each tuple $(p, a, \oout, \mathtt{x})\in Q \times \clS \times \oalph \times \Gamma$ there is at most one $q\in Q$ such that $(p, a, \oout, \mathtt{x}, q)\in\Delta$, 
	%and for each triple  $(p, a, \oout) \in Q \times \noS \times \oalph$ there is at most one $q\in Q$ such that $(p, a, \oout, q) \in \Delta$. 
	On the other hand, we say that $\cA$ is 
	%\emph{input/output unambiguous} (I/O-unambiguous for short) 
	{\it unambiguous} if for every $d\in \Sigma^*$ and every $\nu \in \sem{\cA}(d)$ there is exactly one accepting run $\rho$ of $\cA$ over $d$ such that $\nu = \ann(\rho)$. 
	Note that an 
	%I/O-deterministic 
	deterministic \rt is also 
	%I/O-unambiguous.
	unambiguous. The definition of deterministic is in line with the notion of I/O-deterministic variable automata of~\cite{FlorenzanoRUVV20} and unambiguous is a generalization of this idea that is enough for the purpose of our enumeration algorithm. Actually, one can easily show that for every \rt $\cA$ there exists an equivalent deterministic \rt and, therefore, an equivalent unambiguous \rt. 
	\begin{lemma}\label{ra:det}
		For every \rtname $\cA$ there exists an deterministic \rtname $\cA'$ such that $\sem{\cA}(d) = \sem{\cA'}(d)$ for every $d\in\Sigma^*$.
	\end{lemma}
	
	We are interested on the following enumeration problem for \rts. Let $\bigcal{C}$ be a class of \rt (e.g. deterministic \rt). 
	
	\begin{center}
		\framebox{
			\begin{tabular}{rl}
				\textbf{Problem:} & $\enumraa[\bigcal{C}]$\\
				\textbf{Input:} & a \rt $\cA \in \bigcal{C}$ and $d\in \Sigma^*$ \\
				\textbf{Output:} & Enumerate $\sem{\cA}(d)$
			\end{tabular}
		}
	\end{center}



==> sections/slps.tex <==
%!TEX root = main.tex

	A context-free grammar is a tuple $G = (N,\Sigma,R,S_0)$, where $N$ is the set of non-terminals, $\Sigma$ is the terminal alphabet, $S_0\in N$ is the start symbol and $R\subseteq N \times(N \cup\Sigma)^{+}$ is the set of rules (as a convention, the rule $(A,w) \in R$ is commonly written as $A\to w$). A context-free grammar $S = (N,\Sigma,R,S_0)$ is a \emph{straight-line
program} (SLP) if $R$ is a total function $N\to(N \cup\Sigma)^{+}$ and the directed graph $(N, \{(A,B)\mid (A,w) \in R \text{ and } B\text{ appears in } w\})$ is acyclic. 
For every $A \in N$, let $\derst_S(A)$ be the unique $w \in (N \cup\Sigma)^{+}$ such that $(A,w) \in R$, and for every $a \in \Sigma$ let $\derst_S(a) = a$.
\cristian{Yo cambiaria ese $\derst_S$, por extender $R$. Ya que $R$ es una función, creo que naturalmente se extiende y no necesitas símbolos nuevos.}
%we also call $A \to \derst_S(A)$ {\em the rule for} $A$. 
For an SLP $S = (N,\Sigma,R,S_0)$, we extend $\derst_S$ to a morphism $(N \cup\Sigma)^{+}\to(N \cup\Sigma)^{+}$ by defining $\derst_S(\alpha_1 \ldots \alpha_n) = \derst_S(\alpha_1)\cdot \ldots \cdot \derst_S(\alpha_n)$, where $\alpha_i \in (N \cup\Sigma)$, for $i\in[1,n] $. Furthermore, we define $\str_S(\alpha) = \alpha$ if $\alpha\in\Sigma^+$, and $\str_S(\alpha) = \str_S(\derst_S(\alpha))$ if $\alpha\in (N\cup\Sigma)^+\setminus\Sigma^+$. By our definition of SLP, $\str_S(A)$ is in $\Sigma^+$ (in particular, it is finite), and uniquely defined for each $A\in N$. We will sometimes write the function $\str_S$ as $\str$ if $S$ is obvious from the context.
%Furthermore, for every $\alpha \in (N \cup\Sigma)^{+}$, we set $\derst^1_S(\alpha) = \derst_S(\alpha)$, $\derst^k_S(\alpha) =
%\derst_S(\derst^{k-1}_S (\alpha))$, for every $k \geq 2$, and $\mathfrak{D}_S(\alpha) = \derst^{|N|}_S (\alpha)$ is the derivative of $\alpha$. By definition, $\mathfrak{D}_S(\alpha) \in \Sigma^+$ for every $\alpha \in (N \cup\Sigma)^{+}$. 

\cristian{Sacar estos resultados y poner la definición principal del problema con Annotated Automata y ejemplos.}

We define the size of an SLP $S$, noted by $|S|$, as the size of its set of non-terminals $N$.
	
	\begin{lemma}\label{slp:sizes}
		Given an SLP $S$, we can compute the values of $|\str(A)|$ for all non-terminals $A$ in $S$ in time $\bigcal{O}(|S|)$.		
	\end{lemma}

%\cristian{Quizás es bueno definir que es el tamaño $|S|$.}

%\begin{lemma}
%	Let $S$ be a SLP for a string $w$ and let $M$ be a regular automaton with state set $Q$. We can check whether $d\in L(M)$ in time $\bigcal{O}(|S| \cdot |Q|^3)$.
%\end{lemma}



From now on, we assume that all SLPs are in Chomsky normal form, due to the following result:

\begin{theorem}[SLP Balancing theorem]
	There is a $c\in\nat$ such that any given SLP $S$ for string $w$ can be transformed in time $\cO(|S|)$ into a SLP $S'$ for $w$ in Chomsky normal form with $|S'| \leq c\cdot|S|$.
\end{theorem}

%\cristian{Es necesario esta suposición? Quizás para lo nuestro lo podemos hacer directamente. }

